Uncovering Factor Level Preferences to Improve Human-Model Alignment

Large language models (LLMs) often exhibit tendencies that diverge from human preferences, such as favoring certain writing styles or producing overly verbose outputs. While crucial for improvement, identifying the factors driving these misalignments remains challenging due to existing evaluation methods' reliance on coarse-grained comparisons and lack of explainability. To address this, we introduce PROFILE, an automated framework to uncover and measure factor-level preference alignment of humans and LLMs. Using PROFILE, we analyze preference alignment across three key tasks: summarization, instruction-following, and document-based QA. We find a significant discrepancy: while LLMs show poor factor-level alignment with human preferences when generating texts, they demonstrate strong alignment in discrimination tasks. We demonstrate how leveraging the identified generation-discrimination gap can be used to improve LLM alignment through multiple approaches, including fine-tuning with self-guidance. Our work highlights the value of factor-level analysis for identifying hidden misalignments and provides a practical framework for improving LLM-human preference alignment.

==> Figure/Addition_RM.tex <==
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{Figure/RM_LLM.pdf}
%     \caption{Kendall Tau correlations comparing the alignment of Reward Model (RM) preferences with LLMs trained using that RM on the summarization task for different RM sizes (13B and 70B).}
%     \label{fig:RM_LM_align}
% \end{figure}

% % \begin{table}[]
% \begin{tabular}{@{}c|r|rr@{}}
% \toprule
% RM-based & \multicolumn{1}{c|}{RM} & \multicolumn{1}{c}{LLMeval} & \multicolumn{1}{c}{LLMgen} \\ \midrule
% RM-13b   & 0.62                    & 0.3                         & -0.25                      \\
% RM-70b   & \textbf{0.65}           & \textbf{0.38}               & \textbf{-0.02}             \\ \bottomrule
% \end{tabular}
% \end{table}
% \begin{wrapfigure}{r}{0.5\textwidth}
%     \vspace{-4mm}
%     \includegraphics[width=0.5\textwidth]{Figure/RM_LLM.pdf}
%     \vspace{-3mm}
% \caption{Factor-level preference alignment($\tau$) of human preferences with Reward Model (RM) preferences and LLMs trained with that RM on the summarization task.}
% \label{fig:RM_LM_align}
% \vspace{-8mm}
% \end{wrapfigure}

\begin{figure}[ht]
\centering
\includegraphics[width=\columnwidth]{Figure/RM_LLM.pdf}
    \caption{Factor-level preference alignment($\tau$) of human preferences with Reward Model (RM) preferences and LLMs trained with that RM on the summarization task.}
    \label{fig:RM_LM_align}
\end{figure}


==> Figure/Rank_doc.tex <==
\begin{figure*}[tp]
% \begin{figure*}[ht]
    \centering
    % Subfigure 3

        \includegraphics[width=0.9\textwidth]{Figure/webgpt_fig_1001.pdf}



    \caption{Comparison of factor-level preference alignment  between humans, GPT-4o, and Gemini-1.5 in Document-based QA. The left bar graphs display \textit{factor scores} ($\tau_{14}$) for selected factors. The right tables show the rankings of all factors for each task. Notably, both models consistently rank `length' as the top factor across tasks, while human preferences vary by task.}
            \label{fig:web_main}
\end{figure*}

==> Figure/Rank_help.tex <==


\begin{figure}[htbp]
    \centering
    % First subfigure
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/Rank_help_graph.pdf}
        \caption{Caption for Figure 1}
        \label{fig:subfig1}
    \end{subfigure}
    \hfill
    % Second subfigure
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/Rank_help_tab.pdf}
        \caption{Caption for Figure 2}
        \label{fig:subfig2}
    \end{subfigure}
    
    \caption{Overall caption for both subfigures}
    \label{fig:mainfig}
\end{figure}




==> Table/Addition_eval_improv.tex <==
% \begin{wraptable}{r}{0.5\textwidth} 
% \vspace{-4mm}
% \centering
% \small
% \begin{tabular}{@{}llll@{}}
% \toprule
%                  & \begin{tabular}[c]{@{}l@{}}Base.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Guide$_{Rand}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Guide$_{Mis}$\end{tabular} \\ \midrule
% Tulu 2.5 &0.529                                                    & 0.532                                                            & \textbf{0.578}                                                               \\
% Mixtral          &0.651                                                    & 0.644                                                              & \textbf{0.664}                                                                \\ \bottomrule
% \end{tabular}
% \caption{Evaluation Agreement(\%) on Baseline and Guide$_{Rand}$, and Guide$_{Mis}$ settings.}
% \label{tab:add_eval_improve}
% \vspace{-3mm}
% \end{wraptable}

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}llll@{}}
\toprule
                 & \begin{tabular}[c]{@{}l@{}}Base.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Guide$_{Rand}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Guide$_{Mis}$\end{tabular} \\ 
\midrule
Tulu 2.5         & 0.529                                          & 0.532                                                  & \textbf{0.578}                                        \\
Mixtral          & 0.651                                          & 0.644                                                  & \textbf{0.664}                                        \\
\bottomrule
\end{tabular}
\caption{Evaluation Agreement(\%) on Baseline, Guide$_{Rand}$, and Guide$_{Mis}$ settings.}
\label{tab:add_eval_improve}
\end{table}



==> Table/experiment_generation_prompt.tex <==
\begin{tcolorbox}
[colback=white,colframe=gray!50!black,title=Prompt for Summary Generation]
\small
A good summary is a shorter piece of text that captures the essence of the original. It aims to accomplish the same purpose and convey the same key information as the original post. Your job is to generate five summaries that would each get a score of 1,2,3,4 and 5.\\
TITLE: \{TITLE\}\\
POST: \{CONTENT\}\\
Generate five summaries that would each get a score of 1,2,3,4 and 5.
\label{tab:summary_gen_example}
\end{tcolorbox}

==> Table/main_result_1_summ.tex <==
\begin{table}[htbp]
    \centering
    \begin{subtable}[t]{0.38\textwidth}
        \centering
        \begin{tabular}{rrr}
            \toprule
            Rank & Favored Factors & $\tau$ \\ \midrule
            1 & \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} intent-align} & 0.596 \\
            2 & \cellcolor[HTML]{3C78D8}formality-align & 0.594 \\
            3 & \cellcolor[HTML]{6D9EEB}atomic\_num & 0.328 \\
            4 & src\_cov & 0.269 \\
            5 & \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.257 \\
            6 & coherence & 0.18 \\
            7 & off-focus & 0.05 \\
            8 & hallucination & -0.037 \\
            9 & fluency & -0.072 \\
            10 & \cellcolor[HTML]{C9DAF8}novel\_word\_ratio & -0.052 \\ \bottomrule
        \end{tabular}
    \caption{Human}
    \end{subtable}%
    \hfill
    \begin{subtable}[t]{0.3\textwidth}
        \centering
        \begin{tabular}{rr}
            \toprule
            Favored Factor & $\tau$ \\ \midrule
            \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.978 \\
            \cellcolor[HTML]{6D9EEB}atomic\_num & 0.836 \\
            src\_cov & 0.765 \\
            coherence & 0.488 \\
            \cellcolor[HTML]{C9DAF8}novel\_word\_ratio & 0.472 \\
            \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} intent-align} & 0.171 \\
            \cellcolor[HTML]{3C78D8}formality-align & 0.140 \\
            hallucination & 0.088 \\
            fluency & -0.038 \\
            off-focus & -0.049 \\ \bottomrule
        \end{tabular}
    \caption{GPT-4o}
    \end{subtable}%
    \hfill
    \begin{subtable}[t]{0.3\textwidth}
        \centering

        \begin{tabular}{rr}
            \toprule
            Favored Factor & $\tau$ \\ \midrule
            \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.906 \\
            \cellcolor[HTML]{6D9EEB}atomic\_num & 0.721 \\
            src\_cov & 0.625 \\
            \cellcolor[HTML]{C9DAF8}novel\_word\_ratio & 0.560 \\
            \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} intent-align} & 0.153 \\
            coherence & 0.149 \\
            hallucination & 0.039 \\
            \cellcolor[HTML]{3C78D8}formality-align & 0.031 \\
            off-focus & -0.013 \\
            fluency & -0.089 \\ \bottomrule
        \end{tabular}
    \caption{Gemini-1.5-Flash}
    \end{subtable}
    \caption{ (Option 1. w/rank) Most Favored Factors of Human, GPT-4o, and Gemini 1.5 Flash in Summarization Task.}
    \label{tab:my-table}
\end{table}






\begin{table}[htbp]
    \centering
    \begin{subtable}[t]{0.33\textwidth}
        \centering

        \begin{tabular}{cr}
            \toprule
            Favored Factor & $\tau$ \\ \midrule
            \rowcolor[HTML]{C9DAF8} intent-alignment & 0.596 \\
            \rowcolor[HTML]{D9D2E9} formality-alignment & 0.594 \\
            \rowcolor[HTML]{FCE5CD} atomic\_num & 0.328 \\
            src\_cov & 0.269 \\
            \rowcolor[HTML]{E06666} word\_len & 0.257 \\
            coherence & 0.180 \\
            off-focus & 0.050 \\
            hallucination & -0.037 \\
            fluency & -0.072 \\
            \rowcolor[HTML]{FF9900} novel\_word\_ratio & -0.167 \\
            \bottomrule
        \end{tabular}
        \caption{Human}
        \label{tab:human_summary_feature}
    \end{subtable}%
    \hfill
    \begin{subtable}[t]{0.33\textwidth}
        \centering

        \begin{tabular}{c r}
            \toprule
            Favored Factor & $\tau$ \\ \midrule
            \rowcolor[HTML]{E06666} word\_len & 0.978 \\
            \rowcolor[HTML]{FCE5CD} atomic\_num & 0.836 \\
            src\_cov & 0.765 \\
            coherence & 0.488 \\
            \rowcolor[HTML]{FF9900} novel\_word\_ratio & 0.472 \\
            \rowcolor[HTML]{C9DAF8} intent-alignment & 0.171 \\
            \rowcolor[HTML]{D9D2E9} formality-alignment & 0.140 \\
            hallucination & 0.088 \\
            fluency & -0.038 \\
            off-focus & -0.049 \\
            \bottomrule
        \end{tabular}
        \caption{GPT-4o}
        \label{tab:gpt-4o_summary_features}
    \end{subtable}%
    \hfill
     \begin{subtable}[t]{0.33\textwidth}
        \centering
        \begin{tabular}{c r}
            \toprule
            Favored Factor & $\tau$ \\ \midrule
            \rowcolor[HTML]{E06666} word\_len & 0.906 \\
            \rowcolor[HTML]{FCE5CD} atomic\_num & 0.721 \\
            src\_cov & 0.625 \\
            \rowcolor[HTML]{FF9900} novel\_word\_ratio & 0.560 \\
            \rowcolor[HTML]{C9DAF8} intent-alignment & 0.153 \\
            coherence & 0.149 \\
            hallucination & 0.039 \\
            \rowcolor[HTML]{D9D2E9} formality-alignment & 0.031 \\
            off-focus & -0.013 \\
            fluency & -0.089 \\
            \bottomrule
        \end{tabular}
        \caption{Gemini-1.5-Flash}
        \label{tab:gemini_15_flash_summary_features}
    \end{subtable}
    \caption{(Option 2. w/o rank) Most Favored Factors of Human, GPT-4o, and Gemini 1.5 Flash in Summarization Task.Summary Features Comparison}
    \label{tab:summary_features_comparison}
\end{table}







==> Table/main_result_1_tot.tex <==
\begin{table}[htbp]
    \centering
    % First Main Subtable: Summarization Task
    \begin{subtable}[t]{\textwidth}
        \centering

        % Human, GPT-4o, Gemini-1.5-Flash
        \begin{subtable}[t]{0.32\textwidth}
            \centering
            \begin{tabular}{rr}
                \toprule
                Favored Factor & $\tau$ \\ \midrule
                \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} intent-align} & 0.596 \\
                \cellcolor[HTML]{3C78D8}formality-align & 0.594 \\
                \cellcolor[HTML]{6D9EEB}atomic\_num & 0.328 \\
                src\_cov & 0.269 \\
                \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.257 \\
                coherence & 0.180 \\
                off-focus & 0.050 \\
                hallucination & -0.037 \\
                fluency & -0.072 \\
                \cellcolor[HTML]{FF9900} novel\_word\_ratio & -0.167 \\ \bottomrule
            \end{tabular}
        \caption*{(i) Human}
        \end{subtable}
        \hfill
        \begin{subtable}[t]{0.32\textwidth}
            \centering
            \begin{tabular}{rr}
                \toprule
                Favored Factor & $\tau$ \\ \midrule
                \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.978 \\
                \cellcolor[HTML]{6D9EEB}atomic\_num & 0.836 \\
                src\_cov & 0.765 \\
                coherence & 0.488 \\
                \cellcolor[HTML]{FF9900} novel\_word\_ratio & 0.472 \\
                \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} intent-align} & 0.171 \\
                \cellcolor[HTML]{3C78D8}formality-align & 0.140 \\
                hallucination & 0.088 \\
                fluency & -0.038 \\
                off-focus & -0.049 \\ \bottomrule
            \end{tabular}
       \caption*{(ii) GPT-4o}
        \end{subtable}
        \hfill
        \begin{subtable}[t]{0.32\textwidth}
            \centering
            \begin{tabular}{rr}
                \toprule
                Favored Factor & $\tau$ \\ \midrule
                \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.906 \\
                \cellcolor[HTML]{6D9EEB}atomic\_num & 0.721 \\
                src\_cov & 0.625 \\
                \cellcolor[HTML]{FF9900} novel\_word\_ratio & 0.560 \\
                \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} intent-align} & 0.153 \\
                coherence & 0.149 \\
                hallucination & 0.039 \\
                \cellcolor[HTML]{3C78D8}formality-align & 0.031 \\
                off-focus & -0.013 \\
                fluency & -0.089 \\ \bottomrule
            \end{tabular}
       \caption*{(iii) Gemini-1.5-Flash}
        \end{subtable}
        \caption{Summarization Task}
    \end{subtable}
    \\
    % Second Main Subtable: SHP-2 Task
    \begin{subtable}[t]{\textwidth}
        \centering

        \begin{subtable}[t]{0.32\textwidth}
            \centering
            \begin{tabular}{rr}
                \toprule
                Favored Factor & $\tau$ \\ \midrule
                \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive}   & 0.21 \\
                \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.18 \\
                \cellcolor[HTML]{6D9EEB}atomic\_num                        & 0.15 \\
                \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len}   & 0.14 \\
                fluency                                                    & 0.10 \\
                coherent                                                   & 0.09 \\
                misinformation                                             & 0.07 \\
                hallucination                                              & 0.06 \\
                off-focus                                                  & -0.02 \\ \bottomrule
            \end{tabular}
        \caption*{(i) Human}
        \end{subtable}
        \hfill
        \begin{subtable}[t]{0.32\textwidth}
            \centering
            \begin{tabular}{rr}
                \toprule
                Favored Factor & $\tau$ \\ \midrule
                \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len}   & 0.96 \\
                \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.90 \\
                \cellcolor[HTML]{6D9EEB}{\color[HTML]{000000} atomic\_num} & 0.86 \\
                coherent                                                   & 0.73 \\
                \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive}   & 0.55 \\
                fluency                                                    & 0.10 \\
                off-focus                                                  & 0.03 \\
                misinformation                                             & -0.13 \\
                hallucination                                              & -0.21 \\ \bottomrule
            \end{tabular}
            \caption*{(ii) GPT-4o}
        \end{subtable}
        \hfill
        \begin{subtable}[t]{0.32\textwidth}
            \centering
            \begin{tabular}{rr}
                \toprule
                Favored Factor & $\tau$ \\ \midrule
                \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len}   & 0.92 \\
                \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.74 \\
                \cellcolor[HTML]{6D9EEB}{\color[HTML]{000000} atomic\_num} & 0.57 \\
                coherent                                                   & 0.51 \\
                \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive}   & 0.50 \\
                hallucination                                              & 0.09 \\
                misinformation                                             & 0.06 \\
                off-focus                                                  & 0.01 \\
                fluency                                                    & -0.09 \\ \bottomrule
            \end{tabular}
         \caption*{(iii) Gemini-1.5-Flash}
        \end{subtable}
        \caption{SHP-2 Task}

    \end{subtable}
    \\
    % Third Main Subtable: WebGPT Task
    \begin{subtable}[t]{\textwidth}
        \centering
        
        \begin{subtable}[t]{0.32\textwidth}
            \centering
            \begin{tabular}{rrr}
                \toprule
                Favored Factor & $\tau_{14}$ \\ \midrule
                \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive}   & 0.36 \\
                \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len}   & 0.09 \\
                \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.09 \\
                atomic\_num                                                & 0.07 \\
                \cellcolor[HTML]{FF9900}{\color[HTML]{FFFFFF} coherent}                                                   & 0.07 \\
                fluency                                                    & 0.04 \\
                misinformation                                             & -0.00 \\
                off-focus                                                  & -0.02 \\
                novel\_word\_ratio                                         & -0.05 \\
                hallucination                                              & -0.14 \\ \bottomrule
            \end{tabular}
        \caption*{Human}
        \end{subtable}
        \hfill
        \begin{subtable}[t]{0.32\textwidth}
            \centering
            \begin{tabular}{rr}
                \toprule
                Favored Factor & $\tau_{14}$ \\ \midrule
                \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.97 \\
                \cellcolor[HTML]{FF9900}{\color[HTML]{FFFFFF} coherent} & 0.87 \\
                \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive} & 0.41 \\
                \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.18 \\
                fluency & 0.17 \\
                novel\_word\_ratio & 0.09 \\
                atomic\_num & 0.09 \\
                off-focus & 0.03 \\
                misinformation & -0.07 \\
                hallucination & -0.20 \\ \bottomrule
            \end{tabular}
        \caption*{GPT-4o}
        \end{subtable}
        \hfill
        \begin{subtable}[t]{0.32\textwidth}
            \centering
            \begin{tabular}{rr}
                \toprule
                Favored Factor & $\tau_{14}$ \\ \midrule
                \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.98 \\
                \cellcolor[HTML]{FF9900}{\color[HTML]{FFFFFF} coherent} & 0.77 \\
                \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive} & 0.49 \\
                fluency & 0.30 \\
                helpfulness & 0.18 \\
                misinformation & 0.11 \\
                off-focus & 0.02 \\
                atomic\_num & -0.03 \\
                hallucination & -0.23 \\
                novel\_word\_ratio & -0.35 \\ \bottomrule
            \end{tabular}
        \caption*{Gemini-1.5-Flash}
        \end{subtable}
    \caption{WebGPT Task}
    \end{subtable}
    \caption{Model Correlations Across Tasks with Human, GPT-4o, and Gemini 1.5 Flash}
    \label{tab:combined-table}
    
\end{table}


==> Table/main_resut_1_shp.tex <==
\begin{table}[htbp]
    \centering
    % Subtable 1: Human
    \begin{subtable}[t]{0.38\textwidth}
        \centering
        \begin{tabular}{rrr}
            \toprule
            Rank & Favored Factors & $\tau$ \\ \midrule
            1 & \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive}   & 0.21 \\
            2 & \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.18 \\
            3 & \cellcolor[HTML]{6D9EEB}atomic\_num                        & 0.15 \\
            4 & \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len}   & 0.14 \\
            5 & fluency                                                    & 0.10 \\
            6 & coherent                                                   & 0.09 \\
            7 & misinformation                                             & 0.07 \\
            8 & hallucination                                              & 0.06 \\
            9 & off-focus                                                  & -0.02 \\ \bottomrule
        \end{tabular}
        \caption{Human}
    \end{subtable}%
    \hfill
    % Subtable 2: GPT-4o
    \begin{subtable}[t]{0.3\textwidth}
        \centering
        \begin{tabular}{rr}
            \toprule
            Favored Factor & $\tau$ \\ \midrule
            \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len}   & 0.96 \\
            \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.90 \\
            \cellcolor[HTML]{6D9EEB}{\color[HTML]{000000} atomic\_num} & 0.86 \\
            coherent                                                   & 0.73 \\
            \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive}   & 0.55 \\
            fluency                                                    & 0.10 \\
            off-focus                                                  & 0.03 \\
            misinformation                                             & -0.13 \\
            hallucination                                              & -0.21 \\ \bottomrule
        \end{tabular}
        \caption{GPT-4o}
    \end{subtable}%
    \hfill
    % Subtable 3: Gemini-1.5-Flash
    \begin{subtable}[t]{0.3\textwidth}
        \centering
        \begin{tabular}{rr}
            \toprule
            Favored Factor & $\tau$ \\ \midrule
            \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len}   & 0.92 \\
            \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.74 \\
            \cellcolor[HTML]{6D9EEB}{\color[HTML]{000000} atomic\_num} & 0.57 \\
            coherent                                                   & 0.51 \\
            \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive}   & 0.50 \\
            hallucination                                              & 0.09 \\
            misinformation                                             & 0.06 \\
            off-focus                                                  & 0.01 \\
            fluency                                                    & -0.09 \\ \bottomrule
        \end{tabular}
        \caption{Gemini-1.5-Flash}
    \end{subtable}
    \caption{Most Favored Factors of Human, GPT-4o, and Gemini 1.5 Flash in SHP-2 Task.}
    \label{tab:my-table}
\end{table}


==> Table/main_resut_1_webgpt.tex <==
\begin{table}[htbp]
    \centering
    % Subtable 1: Tau_14 for Human
    \begin{subtable}[t]{0.38\textwidth}
        \centering
        \begin{tabular}{rrr}
            \toprule
            Rank & Favored Factors & $\tau_{14}$ \\ \midrule
            1 & \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive} & 0.36 \\
            2 & \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.09 \\
            3 & \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.09 \\
            4 & atomic\_num & 0.07 \\
            5 & \cellcolor[HTML]{E06666}{\color[HTML]{FFFFFF} coherent} & 0.07 \\
            6 & fluency & 0.04 \\
            7 & misinformation & -0.00 \\
            8 & off-focus & -0.02 \\
            9 & novel\_word\_ratio & -0.05 \\
            10 & hallucination & -0.14 \\ \bottomrule
        \end{tabular}
        \caption{Human}
    \end{subtable}%
    \hfill
    % Subtable 2: Tau_14 for GPT-4o
    \begin{subtable}[t]{0.3\textwidth}
        \centering
        \begin{tabular}{rr}
            \toprule
            Favored Factor & $\tau_{14}$ \\ \midrule
            \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.97 \\
            \cellcolor[HTML]{E06666}{\color[HTML]{FFFFFF} coherent} & 0.87 \\
            \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive} & 0.41 \\
            \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.18 \\
            fluency & 0.17 \\
            novel\_word\_ratio & 0.09 \\
            atomic\_num & 0.09 \\
            off-focus & 0.03 \\
            misinformation & -0.07 \\
            hallucination & -0.20 \\ \bottomrule
        \end{tabular}
        \caption{GPT-4o}
    \end{subtable}%
    \hfill
    % Subtable 3: Tau_14 for Gemini-1.5-Flash
    \begin{subtable}[t]{0.3\textwidth}
        \centering
        \begin{tabular}{rr}
            \toprule
            Favored Factor & $\tau_{14}$ \\ \midrule
            \cellcolor[HTML]{A61C00}{\color[HTML]{FFFFFF} word\_len} & 0.98 \\
            \cellcolor[HTML]{E06666}{\color[HTML]{FFFFFF} coherent} & 0.77 \\
            \cellcolor[HTML]{1C4587}{\color[HTML]{FFFFFF} receptive} & 0.49 \\
            fluency & 0.30 \\
            \cellcolor[HTML]{3C78D8}{\color[HTML]{FFFFFF} helpfulness} & 0.18 \\
            misinformation & 0.11 \\
            off-focus & 0.02 \\
            atomic\_num & -0.03 \\
            hallucination & -0.23 \\
            novel\_word\_ratio & -0.35 \\ \bottomrule
        \end{tabular}
        \caption{Gemini-1.5-Flash}
    \end{subtable}
    \caption{Most Favored Factors of Human, GPT-4o, and Gemini 1.5 Flash in WebGPT Task.}
    \label{tab:my-table}
\end{table}

==> Table/method_taxonomy.tex <==
\begin{table}[htbp]
\centering
\tiny
\begin{tabular}{@{}c|c|c|l@{}}
\toprule
Level 3                        & Level 2                           & Level 1             & Definition                                                                                                                                            \\ \midrule
\multirow{3}{*}{Input-Output}  & \multirow{3}{*}{Relevance}        & Intent-alignment    & Whether the intent of the source and output is the same~\citep{hu-etal-2023-decipherpref}                                                                                               \\ \cmidrule(l){3-4} 
                               &                                   & Receptiveness       & Whether the core question of the input has been answered                                                                                              \\ \cmidrule(l){3-4} 
                               &                                   & Off-focus           & The ratio of atomic facts that are not related to the main focus of the input                                                                         \\ \midrule
\multirow{4}{*}{Source-Output} & \multirow{2}{*}{Consistency}      & Hallucination       & The ratio of atomic facts that align accurately with the original text                                                                                \\ \cmidrule(l){3-4} 
                               &                                   & Source Coverage     & The ratio of atomic facts in the source that appear in the output                                                                                     \\ \cmidrule(l){2-4} 
                               & \multirow{2}{*}{Linguistic Style} & Formality-alignment & Whether the formality of the post and summary is the same (aligned, partially aligned, not aligned)                                                   \\ \cmidrule(l){3-4} 
                               &                                   & Novel words         & The ratio of words in the output that are not used in the source                                                                                      \\ \midrule
\multirow{5}{*}{Output-Only}   & \multirow{2}{*}{Linguistic Style} & Length              & The number of words used in the output                                                                                                                \\ \cmidrule(l){3-4} 
                               &                                   & Fluency             & The quality of individual sentences ~\citep{zhong-etal-2022-towards}                                                                                 \\ \cmidrule(l){2-4} 
                               & \multirow{2}{*}{Informativeness}  & Number of facts     & The number of atomic facts in the output                                                                                                              \\ \cmidrule(l){3-4} 
                               &                                   & Helpfulness         & The ratio of atomic facts that provide additional helpful information~\citep{nakano2021webgpt} \\ \cmidrule(l){2-4} 
                               & Safety                            & Misinformation      & The ratio of atomic facts that include potentially incorrect or misleading information~\citep{xu2021bot}                                                                \\ \midrule
Intra-Output                   & Coherence                         & Coherence           & Whether all the sentences form a coherent body~\citep{zhong-etal-2022-towards}                                                                        \\ \bottomrule
\end{tabular}

\caption{The taxonomy and definitions of the factors.} 
\label{tab:taxonomy}
\end{table}




==> Text/1_Introduction_0516.tex <==
Human preference for a piece of text is inherently multifaceted, influenced by a complex interplay of factors such as fluency, helpfulness, and conciseness. For instance, a desirable summary should be concise and to the point, while \revise{creative writing might prioritize novelty and engaging narrative}. The relative importance of these factors is not static; it often shifts depending on the specific task and context. Despite advancements in large language models (LLMs) that enable them to generate increasingly human-like text, a critical question remains: do these models inherently prioritize these quality factors in a way that aligns with human expectations when they generate responses?

Current models are often optimized using human feedback~\citep{ouyang2022training, rafailov2024direct,song2024preference}, yet the underlying reasons for their generation choices are not well understood. We hypothesize that models may develop implicit biases or prioritization schemes that deviate from human judgment. Specifically, we ask: What factors predominantly influence model-generated outputs? What are their relative weights? More importantly, \textit{how do these model-level priorities differ from those valued by humans across various tasks?}

Prior works~\cite{west2023generative, oh-etal-2024-generative} suggest that a model's ability to generate responses and its ability to discriminate between them are not necessarily aligned. We study whether this is also the case for factor-level preference alignment. Specifically, we observe how models prioritize factors when \textit{judging} existing responses. This is important as LLMs are increasingly used as evaluators, providing feedback that serves as a training signal for improving model performance~\citep{bai2022constitutional, Lee2023RLAIFVR, guo2024direct}
\revise{Then, we see if we can leverage more-aligned setting to ...}

\input{Figure/Main_Figure}
To investigate these questions, we introduce PROFILE (Probing Factors of Influence for Explainability), an automated framework designed to dissect and quantify how individual factors contribute to overall preference. PROFILE allows us to systematically compare what humans value against what models prioritize, moving beyond surface-level quality scores to uncover deeper, factor-level alignments and misalignments.


\input{Figure/pipeline}
Using PROFILE, we measure LLM alignment with human preferences at a factor level across three key preference alignment tasks: summarization, instruction-following, and document-based QA. Our analysis of eight LLMs reveals \revise{a significant divergence in how models and humans weigh different factors during text generation}. 
As illustrated in Figure~\ref{fig:main}, humans exhibit task-dependent preferences; for example, prioritizing conciseness in summarization but responsiveness for instruction-following tasks. In contrast, we find that models often adhere to a more rigid pattern of generating longer for higher quality outputs, regardless of task. Even in summarization, where conciseness is key, models consistently demonstrate a strong preference for generating longer outputs, irrespective of whether increased length contributes positively to the task-specific quality. 
However, these same models demonstrate much stronger alignment in discrimination tasks, with the best model reaching a 0.822 correlation.

% As illustrated in Figure~\ref{fig:main}, humans exhibit task-dependent preferences; for example, prioritizing conciseness in summarization but perhaps elaboration in explanatory tasks. In contrast, we find that models often adhere to a more rigid pattern. Across diverse tasks, including summarization where brevity is key, models consistently demonstrate a strong preference for generating longer outputs, irrespective of whether increased length contributes positively to the task-specific quality. This ``length bias'' is just one example of how models' internal generation preferences can be misaligned with human expectations.


\revise{ADD:why we look at evaluation} Interestingly, our investigation further reveals that these same models exhibit a closer alignment with human factor preferences when they are tasked with evaluating text rather than generating it. This observation suggests that models possess a more nuanced understanding of quality than their generation behavior alone might indicate. 
% Building on this insight, we demonstrate methods to mitigate generation-time misalignment by leveraging the model's more human-aligned evaluation capabilities to guide its generation process.}
Finally, we empirically show that leveraging this gen-eval gap can improve generation-time alignment through experiments with (i) self-guided SFT, (ii) improvement with LLM-evaluator's feedback.

% We leverage this generation-evaluation gap to enhance LLM alignment through (i) supervised fine-tuning with self-evaluation, (ii) improvement with feedback from better-aligned evaluator. 

% First, we show that supervised fine-tuning using self-evaluation effectively narrows this gap, providing empirical support for self-refinement techniques. Second, we show that using feedback from LLM evaluators---which exhibit stronger alignment with human preferences than generators---improves the factor-level alignment of generated outputs.

This work makes the following contributions:
\begin{enumerate}[itemsep=0.5pt, topsep=0.5pt]
    \item We introduce PROFILE, an automated framework for quantifying and comparing factor-level preferences between humans and models. 
    \item We demonstrate through PROFILE that models exhibit systematic misalignments with human preferences in generation, notably a consistent bias towards longer outputs across various tasks.
    \item We demonstrate that the alignment of a model’s generated text improves by leveraging the model’s evaluation ability, which is more aligned with human preferences.
\end{enumerate}
% By providing a deeper understanding of model preferences, PROFILE paves the way for developing LLMs that are not only fluent but also more genuinely aligned with nuanced human values across a spectrum of applications.

==> Text/1_Introduction_new.tex <==
Human preference is inherently multifaceted, influenced by a complex interplay of factors such as fluency, helpfulness, and conciseness. For instance, a desirable summary should be concise and to the point, while creative writing might prioritize novelty and engaging narrative. The relative importance of these factors is not static; it often shifts depending on the specific task and context. Despite advancements in large language models (LLMs) that enable them to generate increasingly human-like text, a critical question remains: do these models inherently prioritize these quality factors in a way that aligns with human expectations when they generate responses?

Current models are often optimized using human feedback, yet the underlying reasons for their generation choices are not well understood.
% Large Language Models (LLMs) are widely recognized for their ability to generate human-level texts, yet they often fail to fully align with human preferences. Despite significant advancements in alignment techniques (e.g., RLHF~\citep{ouyang2022training},  DPO~\citep{rafailov2024direct}), LLMs tend to exhibit biases toward specific writing styles~\citep{das2024under} or generate verbose outputs~\citep{park-etal-2024-disentangling}. 
Previous attempts to understand and improve preference alignment~\citep{ouyang2022training, rafailov2024direct,song2024preference} have primarily relied on coarse-grained approaches, lacking explainability. These methods often focus on identifying which model is preferred overall but do not provide insights into the factors that drive these preferences.
Although some studies analyze human preferences at a finer granularity~\citep{hu-etal-2023-decipherpref,kirk2024prism, scheurer2023training}, a comprehensive comparison with model preferences remains limited. 
% a comparative analysis of how these preferences align with models remains limited. 
% Moreover, existing evaluation approaches often lack scalability and generalizability across diverse tasks due to their dependence on human annotation~\citep{chiang2024chatbot,zheng2023judging}.

\input{Figure/Main_Figure}
% To investigate these questions, we introduce PROFILE (Probing Factors of Influence for Explainability), an automated framework designed to dissect and quantify how individual factors contribute to overall preference. PROFILE allows us to systematically compare what humans value against what models prioritize, moving beyond surface-level quality scores to uncover deeper, factor-level alignments and misalignments.

To address these limitations, we introduce PROFILE (Probing Factors of Influence for Explainability), an automated framework designed to dissect and quantify how individual factors contribute to overall preference. PROFILE allows us to systematically compare what humans value against what models prioritize, moving beyond surface-level quality scores to uncover deeper, factor-level alignments and misalignments.

% a framework that uncovers and quantifies key factors driving both human and model preferences in generation and evaluation. 
% PROFILE systematically analyzes preference alignment by measuring relevant factors' presence in responses, comparing these manifestations between response pairs, and analyzing their alignment with overall response-level preferences. This enables us to determine each factor's influence and compare factor influence rankings between humans and models (Figure~\ref{fig:main}).
% Our framework analyzes pairwise preference data to measure how specific factors manifest in preferred responses and rank the relative influence of different factors,  and compare these rankings between humans and models (Figure~\ref{fig:main}).
% This factor-level understanding provides actionable insights for improving LLM alignment across various tasks and settings.
% , including both generation and evaluation. 
% Furthermore, it is applicable across various tasks and settings, enabling comprehensive analysis of model behavior both as a text generator and as an evaluator.
% This dual-purpose analysis is particularly crucial as LLMs increasingly serve as evaluators that assess and provide feedback on text quality for AI training~\citep{bai2022constitutional, Lee2023RLAIFVR, guo2024direct}.
% enables analysis not only of model generation but also of the evaluations made by human or model judges.
% Applicable across diverse tasks and scenarios, PROFILE facilitates automated analysis of both human and model judgments. 
% Figure~\ref{fig:main} is an illustration of PROFILE framework.

% Using PROFILE, we measure LLM alignment with human preferences at a factor level across three key preference alignment tasks: summarization, instruction-following, and document-based QA. Our analysis of eight LLMs reveals \revise{a significant divergence in how models and humans weigh different factors during text generation}. 
 

Using PROFILE, we conduct a comprehensive investigation of LLM alignment with human preferences at a factor level across three key tasks: summarization, instruction-following, and document-based QA.
Our analysis of eight LLMs reveals a striking discrepancy: in generation tasks, even the best-performing model achieves only a 0.289 correlation with human preferences,
% comparing eight LLMs against human preferences. Our results reveal a significant discrepancy in generation, with the best model achieving only a 0.289 correlation with human preferences, 
often prioritizing length contrary to human preferences. 
However, these same models demonstrate remarkably strong alignment in evaluation tasks, with the best model reaching a 0.822 correlation.
As illustrated in Figure~\ref{fig:main}, humans exhibit task-dependent preferences; for example, prioritizing conciseness in summarization but responsiveness for instruction-following tasks. In contrast, we find that models consistently demonstrate a strong preference for generating longer outputs, irrespective of whether increased length contributes positively to the task-specific quality.
% However, in evaluation, LLMs show surprising alignment, with the best model reaching a 0.822 correlation.  

% With the existing gap between generation and evaluation, we demonstrate that leveraging this gap and factor-level analysis can significantly improve LLM alignment through multiple approaches. 
We leverage this generation-evaluation gap and factor-level insights to enhance LLM alignment through multiple approaches.
First, we show that supervised fine-tuning using self-evaluation effectively narrows this gap, providing empirical support for self-refinement techniques. Second, we show that using feedback from LLM evaluators---which exhibit stronger alignment with human preferences than generators---improves the factor-level alignment of generated outputs.
Finally, we improve evaluation accuracy by incorporating guidance on PROFILE-identified misaligned factors into the instruction for LLM evaluator.
% we find that prompting LLM evaluators with guidance on misaligned factors identified by PROFILE improves overall evaluation accuracy. 
Our findings demonstrate the potential of factor-level analysis and the generation-evaluation gap for improving LLM alignment, opening new directions for future research in alignment techniques.
% These findings suggest both the generation-evaluation gap and factor-level analysis can provide valuable training signals for improving human-LLM alignment. 

% Leveraging these insights, we show that factor level analysis can significantly improve LLM alignment. 
% In the summarization task, we find that prompting LLM evaluators with guidance on misaligned factors identified by PROFILE improves the overall evaluation accuracy. 
% % In the summarization task, guiding LLM evaluators with rubric prompts based on misalignment factors identified by PROFILE enhances overall evaluation agreement with human judgments. 
% % Additionally, using feedback from LLM evaluators, which align more closely with human preferences than LLMs as generators, improves the alignment of model generations with human preferences at the factor level. 
% Using feedback from LLMs as evaluators, which exhibit closer alignment to human preferences than LLMs as generators, improves the factor level alignment of model-generated output.
% These findings suggest PROFILE can provide valuable training signals for improving human-LLM alignment.
% going beyond the benefits of fine-grained guidance in methods like  fine-grained RLHF~\citep{wu2023finegrainedhumanfeedbackgives} and LLMRefine~\citep{xu-etal-2024-llmrefine}.
% \\\\
Our contributions are as follows:
% \begin{itemize}[left=0pt]

\begin{enumerate} 
    \setlength{\itemindent}{0em}
    \item We present PROFILE, a framework for quantifying factor-level preference alignment between humans and LLMs. PROFILE is task-agnostic and scalable, requiring no fine-grained annotations.
    % PROFILE is adaptable across tasks, operates without fine-grained human annotations, and enables scalable analysis of both human and LLM in various settings.
    % \textbf{Introducing PROFILE: An Explainable Framework for Preference Analysis}: 
    % We present PROFILE, a framework for analyzing factor level preferences in human-model alignment. PROFILE is adaptable across tasks, operates without fine-grained human annotations, and enables scalable analysis of both human and model judgments.
    \item Using PROFILE, we reveal significant misalignments between human and LLM preferences in generation, contrasting with surprisingly strong alignment in evaluation.
    % even when their overall performance appears strong. Notably, we show that LLMs align more closely with human preferences in evaluation than in generation setting.
    %This highlights the limitations of solely relying on high-level metrics for evaluating preference alignment. 
    % \textbf{Unveiling Factor Preference Misalignment in Generation}: 
    \item We demonstrate that leveraging a model's own evaluation capabilities improves generation alignment through fine-tuning guided by self-evaluation and refinement with explicit evaluator feedback.
    % \item We show that the factor-level insights from PROFILE can improve alignment in both generation and evaluation settings, and LLM's self-feedback using the gap between generation and evaluation can further improve generation alignment. 
    % in both generation and evaluation settings, along with the insights from comparing these settings, can help improve human-LLM alignment.
\end{enumerate}
% \end{itemize}

\input{Figure/pipeline}

==> Text/3_Experiments_new_2.tex <==
\input{Figure/taxonomy}
This section introduces PROFILE, a novel method for automatically quantifying the influence of specific factors on both human and model preferences, revealing \textit{factor-level preferences}. Building on the work of \citet{hu-etal-2023-decipherpref}, which analyzes factors influencing human preferences, PROFILE extends this analysis to assess preference alignment between humans and models by identifying the driving factors behind these preferences.

% PROFILE comprises three key components: (1) a comprehensive taxonomy of fine-grained factors that influence human preferences (\S\ref{sec:factor_taxonomy}), (2) a methodology for quantifying the influence of each factor, enabling the determination of \textit{factor-level preferences} (\S\ref{sec:profile-metric}), and (3) a framework for automatically determining the manifestation of factors in responses (\S\ref{sec:factor_manifestation}).  
PROFILE's versatility across various agents (humans and models), tasks (generation and evaluation), and settings makes it a powerful tool for comprehensive preference alignment analysis.

\subsection{Factor-Level Preferences}
\label{sec:profile-metric}

% Our central question is how well LLMs align with human preferences.  Recognizing the multifaceted nature of human preference, where perceived quality depends on various factors, we aim to uncover these latent preferences by defining a set of factors $\mathcal{F} = \{f_1, f_2, \ldots, f_n\}$ that influence human preferences. Each $f_i$ represents a specific aspect of the text (e.g., fluency, length). We quantify their influence on human preference as \textit{factor-level preferences}, denoted by $\mathbf{f}(\mathcal{R}) = (f_1(\mathcal{R}), f_2(\mathcal{R}), \ldots, f_n(\mathcal{R}))$, where $f_i(\mathcal{R})$ represents the \textit{factor score} of factor $f_i$ on the response set $\mathcal{R}$. We refer to both humans and models as "agents."

To understand how well LLMs align with human preferences, we must acknowledge that human preference is multifaceted.  The perceived quality of a response depends on various factors, which we call \textit{\textbf{preference factors}}. These represent specific aspects of text, such as fluency, length, or word choice.

Each response has a set of \textit{\textbf{factor scores}}, one for each preference factor, representing the strength of that factor in the response. For example, a response might have a high fluency score and a low length score.

\subsection{Operational Definitions}
\label{sec:opr-def}

% We determine factor-level preferences $\mathbf{f}(\mathcal{R})$ by analyzing observable response-level preferences in a pairwise comparison setting. This involves an agent comparing two responses, $r_i$ and $r_j$, and selecting the preferred one (or indicating a tie).
We determine factor scores by analyzing preferences through pairwise comparisons.  An agent (human or model) compares two responses and selects the preferred one or indicates a tie.
This approach reflects how humans often make choices by comparing options directly.

% \paragraph{Pairwise Preferences.} We define the pairwise preference function as: $Pref: \mathcal{R} \times \mathcal{R} \to \{-1, 0, 1\}$, where $Pref(r_i, r_j) = 1$ if $r_i$ is preferred over $r_j$, $-1$ if $r_j$ is preferred over $r_i$, and $0$ for a tie.

\paragraph{Pairwise Preferences.} The outcome of a pairwise comparison is defined as:
$Pref(r_i, r_j) = 1$ if $r_i$ is preferred over $r_j$, $-1$ if $r_j$ is preferred over $r_i$, and $0$ for a tie.


\paragraph{Model Pairwise Preferences.}  We define model preferences operationally through generated responses at different score levels.

\begin{itemize}
    \item \textbf{Generation:} We prompt the model to generate responses corresponding to predefined scores (e.g., 1 to 5), forming $\mathcal{R} = \{r_{score} \mid score \in \{1, 2, 3, 4, 5\}\}$. Pairwise preference in generation, $Pref_{gen}$, is defined by comparing model-assigned scores: $Pref_{gen}(r_i, r_j) = 1$ if $Score(r_i) > Score(r_j)$, and $-1$ if $Score(r_i) < Score(r_j)$.
    \item \textbf{Evaluation:} Given two responses, the model selects the preferred one. $Pref_{eval}(r_i, r_j) = 1$ if the model prefers $r_i$, $-1$ if it prefers $r_j$, and $0$ for a tie.
\end{itemize}

We assume human preferences are consistent across generation and evaluation, as human judgments are always based on evaluating generated outputs.

\paragraph{Pairwise Factor Comparison.}  For each factor $f_k$, we define $M_k: \mathcal{R} \times \mathcal{R} \to \{-1, 0, 1\}$, where $M_k(r_i, r_j) = 1$ if $f_k$ is more manifest in $r_i$, $-1$ if more manifest in $r_j$, and $0$ if equally manifest. For example, if $f_k$ is length and $r_i$ is longer, $M_{length}(r_i, r_j) = 1$.

\subsection{Automatic Factor Manifestation}
\label{sec:factor_manifestation}

To automatically determine $M_k$, we employ three approaches: (i) \textbf{Rule-based:} For objective factors (e.g., Length, Novel Words), we use deterministic algorithms. (ii) \textbf{UniEval-based:} For subjective factors (e.g., Fluency, Coherence), we use UniEval \citep{zhong-etal-2022-towards}. (iii) \textbf{LLM-based:} For factors requiring nuanced judgment (e.g., Intent Alignment, Formality Alignment), we use GPT-4 with carefully designed prompts. This is further divided into response-based and atomic-fact-based extraction.
Details of each method and validation are in Appendix~\ref{sec:appendix_profile}.

\subsection{Quantifying Factor Influence and Alignment}
\label{sec:profile-metric}

We quantify the influence of each factor (factor score) using $\tau_{14}$, a variation of Kendall's correlation suited for handling ties \citep{deutsch-etal-2023-ties}.  For each factor $f_k$:

\[
\tau_{14}(f_k) = \frac{|C_k| - |D_k|}{|C_k| + |D_k| + |T_k|},
\]

where $C_k$ is the count of concordant pairs (preference and factor manifestation agree), $D_k$ is the count of discordant pairs (disagree), and $T_k$ is the count of ties.

\[
C_k = \sum_{r_i, r_j \in \mathcal{R}, i<j} \mathbbm{1}[Pref(r_i, r_j) \cdot M_k(r_i, r_j) = +1]
\]
\[
D_k = \sum_{r_i, r_j \in \mathcal{R}, i<j} \mathbbm{1}[Pref(r_i, r_j) \cdot M_k(r_i, r_j) = -1]
\]

$T_k$ is defined differently for each setting:

\begin{itemize}
    \item \textbf{Generation:} $T_k$ counts ties at the factor level ($M_k(r_i, r_j) = 0$).
    \item \textbf{Evaluation:} $T_k$ counts ties in preference ($Pref(r_i, r_j) = 0$). Ties at the factor level are removed.
\end{itemize}

A positive $\tau_{14}$ indicates a positive factor influence, a negative value indicates a negative influence, and a value near zero implies minimal influence.

Agent's factor-level preferences are rankings of factors based on their $\tau_{14}$ scores. We use Spearman's $\rho$, Kendall's $\tau_b$, and Pearson's $r$ to quantify the alignment between human and model factor-level preferences.

\subsection{Factor Taxonomy}
\label{sec:factor_taxonomy}
We present a unified taxonomy that systematically categorizes the factors determining preference alignment between humans and AI models across text generation tasks. 
Addressing the lack of a unified framework and inconsistent terminology in existing literature, we incorporate evaluation factors from various tasks, including summarization, helpful response generation, question answering, and instruction following.
% We consolidated definitions from ~\citet{fu2024gptscore, hu-etal-2023-decipherpref, zhong-etal-2022-towards, fabbri2021summeval} for summarization, \citet{glaese2022improving, ye2024flask, nakano2021webgpt} for helpfulness and document-based QA tasks.

To develop this comprehensive framework, we consolidated evaluation metrics and definitions from multiple seminal works. For summarization-specific factors, we drew from~\citet{fu2024gptscore, hu-etal-2023-decipherpref, zhong-etal-2022-towards, fabbri2021summeval}. For helpfulness and document-based question answering, we incorporated categories from \citet{glaese2022improving, ye2024flask, nakano2021webgpt}.
The complete taxonomy is detailed in Table~\ref{tab:taxonomy}.

==> Text/4_Fine-grained_Feature.tex <==
We introduce PROFILE, a novel method for automatically quantifying the influence of specific factors on both human and model preferences, revealing \textit{factor-level preferences}. Building on the work of \citet{hu-etal-2023-decipherpref}, which analyzes factors influencing human preferences, PROFILE extends this analysis to assess preference alignment between humans and models by identifying the driving factors behind these preferences. 

We first establish a comprehensive taxonomy of fine-grained factors to guide the selection of appropriate factor sets \(\mathcal{F}\) for the tasks (\S~\ref{sec:factor_taxonomy}). We then detail methods for quantifying the influence of each factor, \( f_i( \mathcal{R}) \), enabling us to determine \textit{factor-level preferences} for each agent and analyze their alignment (\S~\ref{sec:profile-metric}). PROFILE's versatility across various agents, tasks, and settings (generation and evaluation) makes it a powerful tool for comprehensive preference alignment analysis.

\subsection{Quantification of Human-Model Preference Alignment}
\label{sec:profile-metric}
This section outlines the process of quantifying \textit{factor-level preferences} and measuring {the alignment of these preferences between humans and the model. First, we calculate \textit{factor score} \(f_i(\mathcal{R})\) by comparing the pairwise preference (\(Pref\)) with the factor-specific pairwise comparison (\(M_k\)) across the set of all possible response pairs in the dataset. These scores are then used to rank the factors, and the alignment between human and model preferences at the factor level is quantitatively evaluated based on these rankings.}

\noindent\textbf {Automatically Determining Factor Manifestation}
To analyze the manifestation of our factors in model and human-preferred responses and 
determine $M_k$, we develop an automatic factor extraction framework. We employ three approaches based on the objectivity of each factor:
(i) Rule-based: For straightforward, objective factors, we use deterministic algorithms. $\mathsf{Length}$ and $\mathsf{Novel\:Words}$ are extracted this way. (ii) UniEval-based: For inherently subjective factors ($\mathsf{Fluency}$ and $\mathsf{Coherence}$), we use the well-established UniEval metric~\citep{zhong-etal-2022-towards}. UniEval is a learned metric that provides scores of range 0-1 for various aspects of text quality. 
% $\mathsf{Fluency}$ and $\mathsf{Coherence}$ are extracted this way.
% achieving around 80\% accuracy in validation by the authors. This approach is further divided into atomic-fact-based and response-based extraction depending on the factor's granularity. 
(iii) LLM-based: For factors that rely on objective criteria but require more nuanced judgment, we use GPT-4o with carefully designed prompts. This approach is further divided into ``response-based'' ($\mathsf{Intent\:Alignment}$ and $\mathsf{Formality\:Alignment}$) and ``atomic-fact-based'' (the remaining seven) extraction depending on the level of detail needed for each factor.
By combining these three approaches, our framework captures a wide range of factors with appropriate levels of objectivity.
The specific details of the implementation of each method and validation of LLM-based extractions can be found in Appendix~\ref{sec:appendix_profile}.
% \paragraph{Ranking Correlation}
% kendall tau a
% kendall tau b : tau\_b = (P - Q) / sqrt((P + Q + T) * (P + Q + U))
% this one is used for our ranking correlation
% there are variations and we're using tau 14 (don't need to mention exact formula here) 
% General kendall correlation v. modified kendall correlation
% Concordance, Discordance, Tie 
% + what our setting is
% \paragraph{}
% Pearson Correlation

% \subsubsection{Mathematical Formalization of Factor Influence}

\noindent\textbf {Quantifying Influence of Each Factor.}
To {quantify the influence of each factor, i.e., \textit{factor score}, we use \(\tau_{14}\), a variation of Kendall's correlation proposed by~\citet{deutsch-etal-2023-ties}.}
{This metric is well-suited for handling the distribution of ties, particularly in our setting, where ties arise in only one of the comparison sets used for calculating Kendall’s \(\tau\). Below, we explain the specific ways ties appear in our analysis.}

Since {our analysis relies on pairwise comparisons, we calculate \(\tau_{14}\) for each factor $f_k$ using pairwise concordance and discordance, following the methodology outlined by~\citet{bojar-etal-2017-results}. The metric is defined as:}
\[
\tau_{14}(f_k) = \frac{|C_k| - |D_k|}{|C_k| + |D_k| + |T_k|},
\]
where \(C_k\) is the count of concordant pairs, where the overall preference and the manifestation of factor \(f_k\) agree, \(D_k\) is the count of discordant pairs, where the overall preference and the manifestation of factor \(f_k\) disagree, and \(T_k\) is the count of ties, are handled differently depending on the context. Mathematically, \(C_k\) and \(D_k\) are computed as:
\[
C_k \textstyle= \sum_{r_i, r_j \in R, i<j} \mathbb{1}[Pref(r_i, r_j) \cdot M_k(r_i, r_j) = +1],\]
\[
D_k \textstyle= \sum_{r_i, r_j \in R, i<j} \mathbb{1}[Pref(r_i, r_j) \cdot M_k(r_i, r_j) = -1], 
\]
% \[
% T_k \textstyle= \sum_{r_i, r_j \in R, i<j} 
% \begin{cases} 
% \mathbb{1}[M_k(r_i, r_j) = 0] & \text{in generation setting} \\
% \mathbb{1}[Pref(r_i, r_j) = 0] & \text{in evaluation setting}
% \end{cases}
% \]
where \(\mathbb{1}[\text{condition}]\) is 1 if the condition is true and 0 otherwise. 

{In our experimental setup, the definition of \(T_k\) depends on the specific setting.}
{(1) In the \textbf{generation} setting, no ties exist in response preferences because models do not generate responses with identical scores. Therefore, \(T_k\) is defined as the occurrence of ties at the factor level, which is calculated as the number of instances where \(M_k(r_i, r_j) = 0\).
(2) In the \textbf{evaluation} setting, ties at the factor level (e.g., pairs with the same length) are removed to allow for a clearer analysis of the factor’s influence. In this case, \(T_k\) is the number of occurrences where \((\text{Pref}(r_i, r_j) = 0)\).}

For instance, consider the factor \(M_{length}\), which measures response length. If response \(r_1\) is longer than \(r_2\) (\(M_{length}(r_1, r_2) = 1\)) and the model prefers \(r_1\) (\(Pref(r_1, r_2) = 1\)), this pair is classified as concordant. Conversely, if the model prefers the shorter \(r_1\), the pair is discordant. Evaluating all pairs, a positive factor score indicates a positive influence of the factor, a negative score indicates a negative influence, and a score close to zero implies minimal influence. The magnitude of the score reflects the strength of this influence.

\input{Figure/taxonomy}

\noindent\textbf {Evaluating Factor-Level Preference Alignment.}
An agent's \textit{factor-level preferences} are defined as a ranking of factors based on their scores, where a higher rank and score indicate a stronger influence of that factor on the agent's overall preference. The correlation between human and model rankings reflects their agreement on the relative importance of factors to overall preference, which we use as a measure of factor-level preference alignment between humans and models. We calculate Spearman's \(\rho\), Kendall's \(\tau\)~\footnote{We use Kendall's $\tau_b$~\citep{kendall1945treatment} as the default.}, and Pearson's \(r\) coefficients to quantify this alignment.
% We assume human preferences are consistent across generation and evaluation tasks since human judgments are always based on evaluating model-generated outputs.

\subsection{Taxonomy Design}
\label{sec:factor_taxonomy}
We present a unified taxonomy that systematically categorizes the factors determining preference alignment between humans and AI models across text generation tasks. 
Addressing the lack of a unified framework and inconsistent terminology in existing literature, we incorporate evaluation factors from various tasks, including summarization, helpful response generation, question answering, and instruction following.
% We consolidated definitions from ~\citet{fu2024gptscore, hu-etal-2023-decipherpref, zhong-etal-2022-towards, fabbri2021summeval} for summarization, \citet{glaese2022improving, ye2024flask, nakano2021webgpt} for helpfulness and document-based QA tasks.
To develop this comprehensive framework, we consolidated evaluation metrics and definitions from multiple seminal works. For summarization-specific factors, we drew from~\citet{fu2024gptscore, hu-etal-2023-decipherpref, zhong-etal-2022-towards, fabbri2021summeval}. For helpfulness and document-based question answering, we incorporated categories from \citet{glaese2022improving, ye2024flask, nakano2021webgpt}.
The complete taxonomy is detailed in Table~\ref{tab:taxonomy}.
% \citep{zhong-etal-2022-towards,fabbri2021summeval,hu-etal-2023-decipherpref, fu2024gptscore, ye2024flask,glaese2022improving,nakano2021webgpt}. 
% Our taxonomy comprises 13 distinct factors directly related to preference alignment. 



==> Text/4_PROFILE_2.tex <==
% Human preference is multifaceted, influenced by many factors such as fluency, helpfulness, and output length. To better understand preference alignment between humans and models, we introduce PROFILE, a framework that automatically quantifies how these factors influence preferences. 
% % Building on the work of \citet{hu-etal-2023-decipherpref},
% PROFILE reveals factor-level preferences that help explain factors driving the human-LLM misalignment.
% @은수: 이파트 사람들이 이거 잘 못이해하니까 뒷 내용 바꾸더라도 우리가 계속 review때도 강조한 것들을 첨에 떠먹여주는게 중요할 것 같아요.
PROFILE is a framework designed to uncover and compare the factor-level preferences of humans and language models (Figure~\ref{fig:pipeline}). It enables:

\begin{enumerate}[itemsep=0.5pt, topsep=1pt] 
    \item \textbf{Interpretation} of overall response quality at a fine-grained factor level. It automatically measures how much each factor (e.g., helpfulness, conciseness, length) contributes to overall preference.
    \item \textbf{Comparison of alignment between human and model preferences.} PROFILE provides a quantitative score that serves as a metric for human-model alignment in factor level.
\end{enumerate}

By making these aspects explicit, PROFILE provides a structured way to diagnose and improve alignment between model behavior and human values.
% PROFILE is task-agnostic and scalable, requiring no fine-grained annotations.

\input{Figure/taxonomy}
% \subsection{Framework Overview}
% PROFILE analyzes preference alignment between humans and models through a systematic comparison of how different factors influence their preferences. 
% Framework 순서대로 설명
% First, Preference에 영향을 미치는 set of Factors를 predefine 하고, 각 response에서 그 factor들이 어떻게 manifest 되는지 measure한다(\S~\ref{sec:factor_analysis}).
% Next, pairwise로 responses 간의 factor manifestation을 compare하고 (\S~\ref{sec:pairwise_comparison}), Finally, 그것이 overall preference와 align되었는가 여부를 전체 set of responses에 대해서 measure해서 각 factor의 influence to the overall preference uncover를 한다 (\S~\ref{sec:uncovering_pref}).
To achieve this, PROFILE follows a three-step process:
First, we predefine a set of factors that influence preferences~(Table~\ref{tab:taxonomy}). For each response, we automatically quantify the presence or strength of these factors. 
% This provides a quantifiable representation of each factor for every response.
Next, we compare these factor manifestations between each pair of responses (\S~\ref{sec:pairwise_comparison}).
Finally, we analyze how these pairwise factor differences correlate with the overall preference labels. 
% across all responses
This allows us to infer the influence of each factor on overall preference (\S~\ref{sec:uncovering_pref}) and to assess how closely model preferences align with those of humans at the factor level. 
% Crucially, it also allows us to measure the alignment between human and model preferences at this detailed factor level.


\subsection{Operational Definitions}
We aim to uncover underlying \textit{factor-level} preferences by analyzing observable \textit{response-level} preferences in a pairwise setting, where an agent determines the better of two responses.
% We determine factor-level preferences by analyzing observable response-level preferences in a pairwise comparison setting. This setting refers to a scenario where an agent compares two responses and selects the preferred one.

\paragraph{Pairwise Preferences.} 
We define the overall response-level pairwise preference function $Pref(r_i, r_j)$ for a given pair of responses \(\{r_i, r_j\}\) as: 
\vspace{-3mm}
% \[
% Pref(r_i, r_j) =
% \begin{cases} 
% 1, & \text{if } r_i \text{ is preferred over } r_j \\ 
% -1, & \text{if } r_j \text{ is preferred over } r_i \\ 
% 0, & \text{if there is a tie}
% \end{cases}
% \]

\vspace{-2mm}
\revise{\[
Pref(r_i, r_j) = \operatorname{sign}\!\big(U(r_i) - U(r_j)\big),
\]
where $U$ denotes the value assigned to a response $r$ by the agent (human or model). $Pref(r_i, r_j) = 1$ when $r_i$ is preferred.
}

% \[
% Pref: \mathcal{R} \times \mathcal{R} \to \{-1, 0, 1\},
% \]
% where $Pref(r_i, r_j) = 1$ if response $r_i$ is preferred over response $r_j$; $Pref(r_i, r_j) = -1$ if response $r_j$ is preferred over response $r_i$; and $Pref(r_i, r_j) = 0$ if the preference between $r_i$ and $r_j$ is a tie.
\paragraph{Model Preference in Generation.} 
Models' preference in generation is traditionally defined using log likelihood. $P(x) = \sum_{i=1}^{n} \log P(x_i | x_{<i})$.
While this is a direct measure of generation preference, manipulating logits to obtain distinctive outputs presents a technical challenge, and log probabilities are often inaccessible for closed models.

As an alternative, we use score-based prompting\footnote{This approach is inspired by methods used in constructing training
dataset for LLM-as-a-judge~\citep{kim2023prometheus}.} as a proxy measure of model preference in generation. 
In this approach, we instruct the LLM to generate a response \textit{conditioned on achieving} a target quality score ranging from 1 to 5. We then define the model's preference based on these \textit{target input scores}. For instance, if response \(r_i\) was generated with a higher target score than response \(r_j\), we define that the model ``prefers'' \(r_i\) in this generation context.

To validate whether the score-based prompting approach effectively approximates the models’ intrinsic generation preferences, we conducted an experiment using 100 samples from summarization tasks. Specifically, we prompted open-source models (Llama-3.1-70B and Mixtral) to generate distinct summaries corresponding to target scores ranging from 1 to 5. For each generated summary, we then computed its log probability. We observed a strong Pearson correlation between the target scores and the log probabilities of the generated summaries (Llama-3.1-70B: 0.975; Mixtral: {0.82}; see Figure~\ref{fig:method-valid} in the Appendix for details).

These results suggest that our scoring mechanism serves as an effective proxy for the models’ intrinsic generation preferences, as reflected in their probabilistic outputs.


% We instruct the LLM to generate a response along with a quality score ranging from 1 to 5.
% We operationally define a model's generation preference based on the scores it assigns to the responses. If a model scores response \(r_i\) higher than \(r_j\), we define it that ``prefers'' \(r_i\).  

% We prompt the model to generate responses for scores 1-5 \((\mathcal{R} = {r_{\text{score}} \mid \text{score} \in {1, 2, 3, 4, 5} })\). 
Thus, model preference in generation, \(Pref_{gen}\), is defined by comparing the model-assigned scores \(Score(r_i)\) and \(Score(r_j)\).
\(Pref_{gen}(r_i, r_j)\) is 1 if \(Score(r_i) > Score(r_j)\), and $-1$ if \(Score(r_i) < Score(r_j)\). 
In this score-based generation context, we assume distinct scores for different responses, so a tie (0) case for \(Pref_{gen}\) is not considered.
% This approach is inspired by methods used in constructing training data for the evaluator model, where LLMs are prompted to generate reference outputs for different scores~\citep{kim2023prometheus}.

% \paragraph{Models' Evaluation Preferences.}  We define evaluation preference by having the model directly compare two responses. Evaluation preference, \(Pref_{eval}(r_i, r_j)\), is $1$ if the model prefers \(r_i\), $-1$ if it prefers \(r_j\), and $0$ if they are equally preferable. This pairwise evaluation approach is similar to how LLMs generate preference labels~\citep{Lee2023RLAIFVR}. We assume human preferences remain consistent across generation and evaluation, as human judgment always involves evaluating generated outputs.

\subsection{Analyzing Preference Factors}
\label{sec:factor_analysis}
\noindent\textbf{Taxonomy of Preference Factors.}
To provide a structured framework for analyzing preferences across diverse text generation tasks, we develop a unified taxonomy of fine-grained factors relevant to text quality. 
This taxonomy categorizes the factors influencing preference alignment between humans and LLMs across text generation tasks. 
Addressing the lack of a unified framework and inconsistent terminology in existing literature, we consolidate evaluation factors from diverse tasks, including summarization, instruction following, and question answering. For summarization-specific factors, we draw from \citet{fu2024gptscore, hu-etal-2023-decipherpref, zhong-etal-2022-towards, fabbri2021summeval}. For instruction-following and document-based question answering, we incorporate categories from \citet{glaese2022improving, ye2024flask, nakano2021webgpt}. The complete taxonomy is detailed in Table~\ref{tab:taxonomy}.

\noindent\textbf{Quantifying Factor Manifestation.}
% We employ several approaches to automatically determine factor manifestation $M_f$, depending on the factor's nature: 
% To analyze the manifestation of our factors in model and human-preferred responses and determine $M_f$, we develop an automatic factor extraction framework. 
We employ several approaches to automatically analyze the manifestation of our factors in responses:
(i) \textbf{Rule-based}: For straightforward, objective factors, we use deterministic algorithms. $\mathsf{Length}$ and $\mathsf{Novel\:Words}$ are extracted this way. (ii) \textbf{UniEval-based}: For inherently subjective factors ($\mathsf{Fluency}$ and $\mathsf{Coherence}$), we use the well-established UniEval metric~\citep{zhong-etal-2022-towards}. UniEval is a learned metric that provides scores of range 0-1 for various aspects of text quality. 
(iii) \textbf{LLM-based}: For factors that rely on objective criteria but require more nuanced judgment, we use GPT-4o with carefully designed prompts. This approach is further divided into ``response-based'' ($\mathsf{Intent\:Alignment}$ and $\mathsf{Formality\:Alignment}$) and ``atomic-fact-based'' (the remaining seven) extraction depending on the level of detail needed for each factor.
The specific details of the implementation of each method and validation of LLM-based extractions can be found in Appendix~\ref{sec:appendix_profile}.

\noindent\textbf{Comparing Factors Pairwise.}
\label{sec:pairwise_comparison}
For each pair of responses, we compare factor manifestation. 
For each factor $f$, we define a function $M_f$ to compare factor's manifestation in pairs of responses:
\vspace{-2mm}
% \[
% M_f(r_i, r_j) =
% \begin{cases} 
% 1, & \parbox[t]{0.5\columnwidth}{if \( f \) is more manifest in response \( r_i \)} \\ 
% -1, & \parbox[t]{0.5\columnwidth}{if \( f \) is more manifest in response \( r_j \)} \\ 
% 0, & \parbox[t]{0.5\columnwidth}{if \( f \) is equally manifest in both responses}
% \end{cases}
% \]
\revise{
\[
M_f(r_i, r_j) = \operatorname{sign}\!\big(m_f(r_i) - m_f(r_j)\big),
\]
where $m_f(r)$ is a scalar measurement of factor $f$ in response $r$.
For example, if $m_{length}(r)$ denotes the length of response $r$, 
then $M_{length}(r_i, r_j) = 1$ when $r_i$ is longer than $r_j$.
}
% For example, if \( r_i \) is longer than \( r_j \), then \( M_{length}(r_i, r_j) = 1 \).


% \[M_f: \mathcal{R} \times \mathcal{R} \to \{-1, 0, 1\}\]
% Specifically, $M_f(r_i, r_j) = 1$ if factor $f_k$ is more manifest in response $r_i$; $M_f(r_i, r_j) = -1$ if factor $f_k$ is more manifest in response $r_j$; and $M_f(r_i, r_j) = 0$ if factor $f_k$ is equally manifest in both responses.

\subsection{Uncovering Factor-level Preferences}
\label{sec:uncovering_pref}
\noindent\textbf{Quantifying Factor Influence.}
To quantify each factor's influence (factor score), we analyze the concordance between response-level preferences $Pref(r_i, r_j)$ and factor manifestation $M_f(r_i, r_j) $ across response pairs. 
% For a given factor $f_k$, we measure whether the overall preference aligns with how that factor manifests in the responses. 
We use $\tau_{14}$, a variation of Kendall's correlation proposed by~\citet{machacek-bojar-2014-results}, which is particularly well-suited for handling ties in our analysis setting, where ties arise in only one of the comparison sets used for calculating Kendall’s \(\tau\). 

The metric is defined as:
\begin{equation} \label{eq:factorscore}
\tau_{14}(f) = \frac{|C_f| - |D_f|}{|C_f| + |D_f| + |T_f|,}
\end{equation}
where \(C_f\) is the count of concordant pairs (preference and factor manifestation agree), \(D_f\) is the count of discordant pairs (preference and factor manifestation disagree), and \(T_f\) represents ties. 
In our setting, since models don't generate responses with identical scores, \(T_f\) only counts factor-level ties ($M_f(r_i, r_j) = 0$)
This pairwise comparison reveals how the differences in factor manifestations relate to differences in preference between the two responses.

For instance, consider the factor \(M_{length}\), which measures response length. If response \(r_1\) is longer than \(r_2\) (\(M_{length}(r_1, r_2) = 1\)) and the model prefers \(r_1\) (\(Pref(r_1, r_2) = 1\)), this pair is classified as concordant. Conversely, if the model prefers the shorter \(r_1\), the pair is discordant. Evaluating all pairs, a positive factor score indicates a positive influence of the factor, a negative score indicates a negative influence, and a score close to zero implies minimal influence. The magnitude of the score reflects the strength of this influence.

\paragraph{Comparing Human and Model Preferences.}
Finally, we evaluate \textit{factor-level preference} alignment by comparing human and model factor rankings. We use Spearman’s \(\rho\), Kendall’s \(\tau\)~\footnote{We use Kendall's $\tau_b$~\citep{kendall1945treatment} as the default.}, and Pearson’s \(r\) coefficients to quantify the correlation between these rankings, providing a measure of how well the model's factor priorities align with human values.


==> Text/6_Discussion.tex <==
\label{sec:discussion}
\noindent\textbf{Alignment of Reward Models and Language Models.}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{Figure/Main_figure.pdf}
    \caption{Factor-level preference alignment($\tau$) of human preferences with Reward Model (RM) preferences and LLMs trained with that RM on the summarization task.}
    \label{fig:RM_LM_align}
\end{figure}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/Main_figure.pdf}
    \caption{LLMs often fall short of expectations, but pinpointing \textit{why} is challenging (left panel). PROFILE quantifies the influence of various factors on preferences, revealing the underlying causes of human-model misalignment (right panel).}
    \label{fig:main}
    \vspace{-1mm}
\end{figure*}
\input{Figure/Addition_RM}
To understand whether preference misalignment originates from reward models (RMs), we compare factor-level alignment between RM, their corresponding RLHF-trained LLM, and human preferences in a summarization task.
%In this comparison, higher RM scores are interpreted as indicating a stronger preference.
%We compare the correlation between human preferences and those of both the RMs (used for LLM training) and the LLMs in evaluation and generation. 

Figure~\ref{fig:RM_LM_align} shows the factor-level alignment ($\tau$) between human preferences and those of RMs and LLMs in both generation and evaluation settings. The results indicate that RMs have a stronger alignment with human preferences than LLMs in both settings, implying that misalignment doesn't stem from the RMs themselves. Additionally, the larger 70B RM displays stronger alignment than the smaller 13B RM, suggesting a positive correlation between RM size and alignment suggests a potential link that motivates further investigation.

% RM exhibits a stronger alignment with the LLM in the evaluation setting compared to the generation setting. Furthermore, we observe a consistent trend where larger models (70B) exhibit stronger alignment with the RM than smaller models (13B), suggesting a potential correlation between model size and alignment with RM preferences. However, further investigation is needed to determine the generalizability of these findings.

% \noindent\textbf{Generation-Evaluation Gap.}
% In Section~\ref{sec:eval_alignment}, we observe a surprising difference in factor-level alignment between LLM generation and evaluation, despite both being fundamentally next-token prediction tasks. 
% Our evaluation-guided generation experiments (\S~\ref{sec:application}) show that GPT-4o often critiques its own summaries in ways that contradict its generation preferences. 
% For instance, it criticized ``unnecessary specifics (like the exact ages and the name of the allergy site)'' in its summaries, despite initially prioritizing number of facts and source coverage in generation setting. 
% This seemingly paradoxical behavior supports the effectiveness of using evaluation to guide generation---it's not merely coincidental. Our findings align with previous work by \citet{west2023generative}, which also observes differences in model performance between generation and evaluation tasks. 
% Our study systematically highlights this disparity and shows how leveraging it can improve alignment, pointing to a promising direction for future research.
% In this study, we systematically demonstrate the disparity in generation and evaluation at factor-level preferences and provide preliminary evidence that leveraging this insight can enhance generation alignment. Further investigation into this intriguing behavior and its implications for improving LLMs is a promising avenue for future research.

% In typical settings, language models directly generate responses to questions. However, our experiment employs a unique approach where the model generates responses using a scoring system from 1 to 5. To assess the generalizability of our setting to more conventional ones, we examine which score (1-5) aligns best with ``direct generation'' – responses generated immediately without any specialized prompting.

% We compare various factors of the responses generated through direct generation with those of the responses across the 1-5 score range. For each factor, we rank the scores based on their similarity to the direct generation output. For instance, if score 5 receives rank 1 for the 'novel\_word\_ratio' factor, it indicates that the direct generation results exhibit the closest resemblance to the 'novel\_word\_ratio' value of score 5 responses.

% Our experiments with GPT-4o, Tulu-2.5-ppo-13b-70brm, and LLaMA 3.1 70B reveal that score 5 consistently ranks highest across most factors when compared to direct generation (see Tables~\ref{tab:1st_rank_gpt4o}~\ref{tab:1st_rank_tulu} in the Appendix). This suggests a strong alignment between the model's immediate, unconstrained responses and those associated with score 5 within our scoring framework. This finding implies that our research findings could potentially be generalized to more standard language modeling settings.

% \noindent\textbf{Alignment over latent preference.} As observed in \citep{park-etal-2024-disentangling}, our experiments reveal that under single-score human preference, the model can exhibit false positive optimization by producing overly lengthy outputs and erroneously believing they have achieved higher human preference. This phenomenon is known as reward hacking \citep{skalse2022definingcharacterizingrewardhacking} and is particularly problematic for downstream tasks like summarization, which require concise and accurate responses. PROFILE can quantify latent preferences and identify misalignments at the factor level, such as \(\mathsf{length}\) and \(\mathsf{Intent\:Alignment}\). PROFILE can be used to diagnose latent human preference misalignment and provide training signals to improve alignment at the factor level. Similar to fine-grained RLHF \citep{wu2023finegrainedhumanfeedbackgives}, we can leverage factor-level scores to align the LLM. Additionally, similar to LLMRefine \citep{xu-etal-2024-llmrefine}, we can employ fine-grained guidance to harness the LLM's self-refinement capability for further improvement.
\noindent\textbf{Alignment over Latent Preference.} 
{Our experiments reveal that under single-score human preference, the model can exhibit false positive optimization by producing overly lengthy outputs and misleadingly exhibiting higher alignment scores, similar to \citet{park-etal-2024-disentangling, skalse2022definingcharacterizingrewardhacking}. This is particularly problematic for downstream tasks like summarization, which require concise responses with the original intention well preserved. PROFILE can be used to diagnose latent human preference misalignment and provide training signals to improve alignment at the factor level. Similar to fine-grained RLHF \citep{wu2023finegrainedhumanfeedbackgives}, we can leverage factor-level scores to align the LLM. Additionally, similar to LLMRefine \citep{xu-etal-2024-llmrefine}, we can employ fine-grained guidance to harness the LLM's self-refinement capability for further improvement.}
% As noted in \citep{park-etal-2024-disentangling}, our experiments show that with single-score human preference, models can engage in reward hacking \citep{skalse2022definingcharacterizingrewardhacking} by generating overly lengthy outputs, mistakenly optimizing for perceived human preference. This issue is particularly problematic for downstream tasks like summarization, which require concise and accurate responses. PROFILE helps quantify latent preferences and identify factor-level misalignments, such as \(\mathsf{length}\) and \(\mathsf{Intent\:Alignment}\). By diagnosing these misalignments, PROFILE offers training signals to improve factor-level alignment. Similar to fine-grained RLHF \citep{wu2023finegrainedhumanfeedbackgives} and LLMRefine \citep{xu-etal-2024-llmrefine}, we can use factor-level scores and fine-grained guidance to enhance LLM alignment and self-refinement.

% {\noindent\textbf{Validation of Score-based Generation Approach.}}
% Our research deviates from the typical language model setup by using a 1-5 scoring system for response generation. To assess the {validity} of our approach, we compare responses generated through direct generation (without scoring) with those across the score range {through all summary, helpfulness, and document-based QA tasks}. {In every task,} we found that score 5 consistently aligns best with direct generation responses, based on the fine-grained factors we use, in models like GPT-4o, Tulu 2.5 + PPO (70B RM), and LLaMA 3.1 70B (see Table~\ref{tab:response_score_similarity} in the Appendix~\ref{sec:appendix_generalizability}). This suggests that our scoring framework, specifically score 5, captures the essence of unconstrained language model outputs, implying the potential generalizability of our findings to general settings.



==> Text/9_Reproducibility.tex <==
The datasets and models we use in our study are detailed in \S~\ref{sec:exp-setting}. For more comprehensive descriptions of the datasets and specific versions of the models, please refer to Appendix~\ref{appendix:sec_task} and \ref{appendix:sec_model}. The methodology we employed for factor extraction in our experiments is presented in Appendix~\ref{sec:appendix_profile}, while the prompting configurations set up for the experiments can be found in Appendix~\ref{sec:appendix_prompts} and \ref{sec:appendix_better_align}.
% Appendix~\ref{sec:appendix_factor_level_alignment} and \ref{sec:appendix_generalizability} contains additional experimental results that are not presented in the main paper, offering important insights and extra experiments that can aid in comparing and reproducing our findings.
Appendix~\ref{sec:appendix_factor_level_alignment} and \ref{sec:appendix_generalizability} contain additional experimental results not presented in the main paper. Appendix~\ref{sec:appendix_factor_level_alignment} provides the lists of all factor scores for both generation and evaluation across all three tasks used in the study. Appendix~\ref{sec:appendix_generalizability} presents detailed results regarding the generalizability of our findings in the \S~\ref{sec:discussion}.

==> Text/archive/1_Introduction.tex <==
% Background & Importance 
% A lot of efforts have been made to align large language models (LLMs) with human preferences, e.g., RLHF, DPO,... but models trained with those alignment methods are not quite aligned yet. dissatisfaction often arises from their outputs, deviating from true human preference in subtle factors. 

Despite significant efforts to align large language models (LLMs) with human preferences, such as RLHF~\citep{ouyang2022training} and DPO~\citep{rafailov2024direct}, achieving true alignment remains elusive. 
Users often express dissatisfaction with LLM outputs, highlighting subtle yet significant deviations from human preferences. 
For instance, LLMs often exhibit consistent biases towards specific writing styles~\citep{das2024under}, or produce overly verbose generations~\citep{park-etal-2024-disentangling}, even when those preferences don't align with human judgments.
This misalignment is particularly concerning given the growing trend of using AI-generated feedback as training signals for preference alignment~\citep{bai2022constitutional, Lee2023RLAIFVR, guo2024direct}. 
Given these challenges, it is imperative to ask: \textit{In what ways and to what extent are LLMs aligned with human preferences?}
% Models are even used to evaluate preferences; there is a growing trend of using AI-generated feedback as training signals for preference alignment~\citep{Lee2023RLAIFVR, guo2024direct}. 
% If LLMs are employed as evaluators for training other models, understanding their alignment at a fine-grained level becomes essential.

% This question is yet to be solved. 
Previous studies primarily rely on coarse-grained, comparative approaches, such as assessing which model is preferred overall, without offering insights into the underlying factors driving these preferences. While some attempts have been made to analyze human preferences at a finer granularity (e.g., ~\citet{hu-etal-2023-decipherpref,kirk2024prism}), a comparative analysis of how these factors manifest in and are aligned with model preferences is limited. 
Furthermore, existing approaches often suffer from limited scalability and generalizability across diverse tasks and settings due to their heavy reliance on human annotation (e.g., Chatbot Arena~\citep{chiang2024chatbot}, MT Bench~\citep{zheng2023judging}) or their exclusive focus on generation tasks (e.g., FLASK~\citep{ye2024flask}).

% Current research on human-model preference alignment primarily focuses on holistic evaluations, such as ranking model-generated outputs or assigning overall scores (e.g., Chatbot Arena). However, this approach lacks interpretability, failing to pinpoint the specific factors contributing to preference judgments. 
% Despite efforts to align LLMs, there remains a limited understanding of how specific factors contribute to these discrepancies. This paper argues for a more granular understanding of human-model preference alignment. Furthermore, building on existing research highlighting performance differences between generation and understanding tasks in LLMs~\citep{oh2024generative, west2023generative}, we investigate whether misalignment stems from a failure to learn fine-grained preferences during training or an inability to incorporate these preferences during generation.

\input{Figure/Main_Figure}
% We argue for a more granular understanding of human-model preference alignment to guide the development of LLMs that better reflect human values and expectations.
To this end, we introduce \textbf{PROFILE}, an analytical method designed to measure preference alignment that is applicable to both human and model preferences. 
% across generation and evaluation scenarios. 
PROFILE probes the factors that influence the preferences (e.g., output length, informativeness, helpfulness), quantifies their contributions, and assesses the degree of alignment between human and model preferences through correlation analysis.
% PROFILE enables a deeper analysis of how models align—or fail to align—with human preferences at a granular factor level. 
Using this framework, we explore three primary research questions: (1) Are model generations aligned with human preferences at a human-interpretable factor level?
(2) Given the prevalence of LLMs as judges for preference, do their evaluations align with human judgments at a granular factor level? (3)~\revise{If models exhibit better factor-level alignment in either evaluation or generation, can we leverage their performance in one task to enhance the other?}

% \begin{enumerate}
% \item Are model generations aligned with human preferences at a human-interpretable factor level?
% \item Given the prevalence of LLMs as judges for preference, do their evaluations align with human judgments at a granular factor level?
% \item If models exhibit better factor-level alignment in either evaluation or generation, can we leverage their performance in one task to enhance the other?
% % \item If models are not aligned in the generation, have they failed to learn preferences for fine-grained features, or do they distinguish them but fail to incorporate them during generation?
% \end{enumerate}

To address these questions, we conduct an in-depth analysis of pairwise human judgments from widely used preference datasets, examining both model-generated responses and model evaluations across three distinct tasks: summarization, helpful response generation, and document-based question answering. We compare the preferences of several LLMs, including both open-source and proprietary models, to human preferences at a granular factor level. Our results show that \add{[ADD QUANTITATIVE RESULTS]}, revealing key insights into the alignment and misalignment of human and model preferences in text generation and evaluation.
% We first dissect these judgments to isolate the factors driving human preferences, such as output length, informativeness, fluency, etc. We then investigate how these same factors influence the preferences exhibited by LLMs. Specifically, we quantify the contribution of individual factors to both human and model judgments. By applying techniques like Kendall correlation analysis, we assess the degree of alignment between human and model preferences for each factor. 

Our contributions are as follows:
\begin{itemize}
    \item \textbf{Fine-Grained Analysis of Preference Alignment}: We introduce PROFILE, an explainable framework for analyzing human-model preference alignment, focusing on specific factors influencing judgments.
    \item \textbf{Revealing Misalignment in Generation}: Our analysis demonstrates a significant misalignment between human and LLM preferences for generated text at a fine-grained level. Notably, we find that LLMs consistently over-prioritize length over other factors like informativeness, even when this contradicts human preferences.
    \item \textbf{Leveraging Evaluation for Better Generation Alignment}: While LLMs struggle to \revise{incorporate fine-grained preferences during generation}, they exhibit a stronger capacity to distinguish these factors when evaluating existing text. We demonstrate that leveraging LLMs' superior evaluation capabilities can lead to better-aligned generations. 
    % This suggests a promising direction for improving the alignment of future LLMs.

\end{itemize}

Our findings have several broader implications. Our findings suggest that current training and evaluation methods for preference alignment could benefit from a more explainable, factor-level approach. By understanding the specific aspects where misalignment occurs, we can better target model training to address these gaps and improve overall performance. While models might exhibit different behaviors in generation and evaluation, this distinction presents an opportunity. We can leverage a model's ability to evaluate fine-grained preferences to enhance its generation capabilities, ultimately leading to more human-aligned outputs. 





==> Text/archive/3_Experiments.tex <==
% 1. Models are not aligned in the fine-grained level with human

% 2. Models are more aligned when they evaluate

\subsection{Definition of Preference}
The potential of generative models to produce responses in countless ways highlights the importance of understanding human preferences. Beyond simply ``solving'' the problem, human preference for a model's response is influenced by numerous factors, each contributing to the overall perception of quality. We focus on these ``fine-grained preferences'' to investigate whether models align with them, both in their generation and evaluation capabilities. [ADD: we're looking at binary preference.]

% \paragraph{Hypothesis.}
% Our central hypothesis is that current models do not align with human preferences at the level of fine-grained factors. While models generate responses, they may not consistently reflect the specific features that humans find desirable. We aim to test this hypothesis, and further investigate whether models have learned these preferences but struggle to generate responses that accurately reflect them.

\paragraph{Operational Definitions.}
To answer our research question, we establish clear operational definitions for each key aspect of our investigation:
\begin{itemize}
    \item \textbf{Factor-level Preferences}: These refer to the detailed features present in responses that an agent (human, model) rates as more favorable. These features define what constitutes a "better" response from the agent’s perspective, contributing to overall quality. 
    \item \textbf{Model Preferences in Generation}: To understand how models express these preferences during generation, we use a score-based generation approach. We prompt models to generate responses across varying score levels, assuming that factors favored by the model will become more pronounced in high-scoring responses, while less preferred features will be more evident in low-scoring responses. This approach is inspired by methods used in constructing training data for evaluator models (e.g., ~\citet{kim2023prometheus}).
    \item \textbf{Model Preferences in Evaluation}: We prompt the models to compare two summaries and select the one they deem superior. By analyzing the factors present in the preferred summaries across multiple pairwise comparisons, we can infer the model's implicit preferences during evaluation.
    % Next, to measure whether a model has learned fine-grained human preferences, we assess its ability to evaluate responses based on these preferences. Although whether a model has learned fine-grained human preferences is not defined by some observable output, we can test it by explicitly defining its effects. We measure this by asking: For a given task, can the model distinguish between better answers that differ in fine-grained factors? 
    This setting is similar to how LLMs generate preference labels, as seen in~\citet{Lee2023RLAIFVR}.

\end{itemize}




We assume that human preferences are consistent across generation and evaluation tasks, as human judgment of preferred outputs always stems from evaluating model outputs.


\subsection{Metrics}
\paragraph{Kendall's Tau:} Kendall's Tau is a non-parametric measure of correlation that assesses the strength and direction of association between two variables. It is based on the ranks of data rather than their actual values, making it robust to outliers and non-normal distributions.

\paragraph{Equation of Tau-14:} The general formula for Kendall's Tau-14 (\(\tau_{14}\)) is:
\begin{equation}
    \tau = \frac{(C - D)}{( C + D + T_x)}
\label{eq:tau14}
\end{equation}
where \(C\) is the number of concordant pairs, \(D\) is the number of discordant pairs, and \(T_x\) is the number of ties in the ranks of the variable \math{x}.
\paragraph{Equation of Tau-b:} Kendall's Tau-b (\(\tau_b\)) is a variation that adjusts for ties and is given by:
\begin{equation}
    \tau_b = \frac{(C - D)}{\sqrt{(C + D + T_x)(C + D + T_y)}}
\label{eq:taub}
\end{equation}
where \(T_x\) and \(T_y\) represent the number of ties in the ranks of the two variables respectively.

==> Text/archive/3_Experiments_new.tex <==
% We start by establishing our problem (\S~\ref{sec:pre-def}) and operational definitions(\S~\ref{sec:opr-def}) to address our research questions.
% , experimental setup(\S~\ref{sec:pre-exp}), and 
% \subsection{Problem Definition}
\label{sec:pre-def}
% The potential of generative models to produce responses in countless ways highlights the importance of understanding human preferences.

To address our central question of how well LLMs align with human preferences,
% ``In what ways and to what extent are LLMs aligned with human preferences?'',
we acknowledge the multifaceted nature of human preference where a perceived quality of response depends on various factors.
% We uncover the latent factors by defining a set of factors that influence the overall preference, and measuring how big each contribution is, from observable response-level preferences.
To uncover these latent preferences, we define a set of factors \( \mathcal{F} = \{ f_1, f_2, \ldots, f_n \} \), which influence human preferences. Each \( f_i \) represents a specific aspect of the text (e.g., fluency, length).
We then quantify their influence on human preference as \textit{factor-level preferences}, denoted by \( \mathbf{f}(\mathcal{R}) \).
% We define these factors as a set \( \mathcal{F} = \{ f_1, f_2, \ldots, f_n \} \), where each $f_i$ represents a specific aspect of a response, such as fluency, length, or word choice.
% We quantify the impact of these factors on what we define as the \textit{factor-level preferences}, represented
\[
\mathbf{f}( \mathcal{R}) = (f_1( \mathcal{R} ), f_2( \mathcal{R}), \ldots, f_n( \mathcal{R} )),
\]

where \( f_i(\mathcal{R}) \) represents the influence of each factor (\( f_i \)) on the overall preference across the response set \( \mathcal{R} \). We refer to \( f_i(\mathcal{R}) \) as the \textit{\textbf{factor score}} of factor \( f_i \). We extend this concept to include both humans and models, referring to both as ``agents.''

% We measure $\textbf{f}$ by examining observable response-level preferences.

\subsection{Operational Definitions}
\label{sec:opr-def}
% To determine factor-level preferences $\mathbf{f}( \mathcal{R})$ in generation and evaluation settings, we analyze preferences in \revise{pairs of responses}, which are directly observable. 
% To determine factor-level preferences $\mathbf{f}( \mathcal{R})$ in generation and evaluation settings, we analyze preferences at response level, which are directly observable. 
% Specifically, we use a pairwise preference setting, where preferences are determined by direct comparison.
% Specifically, we experiment with a pairwise preference setting, where preferences are determined by comparing two responses.
% We determine factor-level preferences $\mathbf{f}( \mathcal{R})$ through a pairwise comparison setting, where preferences are directly observed at the response level.

We determine factor-level preferences $\mathbf{f}( \mathcal{R})$ by analyzing observable response-level preferences in a pairwise comparison setting.
This setting refers to a scenario where an agent compares two responses, e.g. \( r_i \) and \( r_j \), and selects the more preferred one (either \( r_i \), \( r_j \), or a tie).
The operational definitions of the pairwise preferences required for this experiment are defined as follows.

\noindent\textbf{Pairwise Preferences.}
We define the pairwise preference function for a pair of two responses as:
    \[
    Pref\textstyle: \mathcal{R} \times \mathcal{R} \to \{-1, 0, 1\}
\]
    where $Pref(r_i, r_j) = 1$ if response $r_i$ is preferred over response $r_j$; $Pref(r_i, r_j) = -1$ if response $r_j$ is preferred over response $r_i$; and $Pref(r_i, r_j) = 0$ if the preference between $r_i$ and $r_j$ is a tie. 
In our experiments, we define model pairwise preferences for both generation and evaluation settings.
% We define the response-level pairwise preference function \(Pref: \mathcal{R} \times \mathcal{R} \to \{-1, 0, 1\}\), where \(Pref(r_i, r_j) = 1\) if \(r_i\) is preferred over \(r_j\), \(Pref(r_i, r_j) = -1\) if \(r_j\) is preferred over \(r_i\), and \(Pref(r_i, r_j) = 0\) for a tie.
    % This function encapsulates how agents evaluate the overall desirability of one response over another.
% \paragraph{Model Preferences in Generation} 
% While models might not possess preferences in the same way humans do, we can operationally define ``model preferences in generation'' through the responses they generate at different score levels. Specifically, we prompt the model to generate a set of responses $\mathcal{R}_s = \{r | S(r) = s\}$ for each score level $s \in \{1, 2, 3, 4, 5\}$, where $S(r)$ be the score assigned by a model to a response $r$. 
% % We hypothesize that factors preferred by the model will be more prominent in higher-scoring responses (larger $s$), while less preferred factors will be more evident in lower-scoring responses (smaller $s$). 
% This approach is inspired by methods used in constructing training data for evaluator models (e.g., ~\citet{kim2023prometheus}).
% \noindent\textbf{Model Preferences in Generation.}
% In our experiment, we address the situations of model generation (\(S = g\)) and evaluation setting (\(S = e\)), and define the model's response-level pairwise preferences for each situation as follows. 

\textbf{Model Pairwise Preferences in Generation.}
While models might not have preferences in the same way humans do, we can operationally define the preferences of a model through the responses it generates at different score levels. 
Specifically, if a model assigns scores of 3 and 5 to two responses, the response with a score of 5 is considered ``preferred" by the model over the response with a score of 3. 
To implement this systematically, we prompt the model to generate responses corresponding to predefined scores ranging from 1 to 5, forming the set \( \mathcal{R} = \{ r_{\text{score}} \mid \text{score} \in \{1, 2, 3, 4, 5\} \}\).
% To implement this systematically, we prompt the model to generate the responses with scores ranging from 1 to 5, \( \mathcal{R} = \{ r_{\text{score}} \mid \text{score} \in \{1, 2, 3, 4, 5\} \}\).} 
% After this, we obtain the response set \( \{r_1, r_2, r_3, r_4, r_5\} \) for each query.
Pairwise Preferences in Generation, \( Pref_{gen} \), is defined by comparing the model-assigned scores \( Score(r_i) \) and \( Score(r_j) \). Specifically, \( Pref_{gen}(r_i, r_j) = 1 \) if \( Score(r_i) > Score(r_j) \) and \( Pref_{gen}(r_i, r_j) = -1 \) if \( Score(r_i) < Score(r_j) \). 
This approach is inspired by methods used in constructing training data for evaluator models~\citep{kim2023prometheus}.
% This captures the model's implicit preferences during the generation process, suggesting that higher-scoring responses capture features the model implicitly favors. 

\noindent\textbf{Model Pairwise Preferences in Evaluation.}
We define model preferences in an evaluation setting, similar to the general approach used to measure human preferences. Given two responses \( r_i \) and \( r_j \), the model {selects} which is the better response.
Pairwise Preferences in Evaluation, \( Pref_{eval}(r_i, r_j) = 1 \) if the model evaluates \( r_i \) as preferable over \( r_j \); \( Pref_{eval}(r_i, r_j) = -1 \) if \( r_j \) is preferred over \( r_i \); and \( Pref_{eval}(r_i, r_j) = 0 \) if the model finds them equally preferable (tie).
This approach, where models make pairwise preference evaluation, is similar to how LLMs generate preference labels~\citep{Lee2023RLAIFVR}. 
Although we extract model preferences separately for evaluation and generation tasks, we assume that human preferences remain consistent across both, as human judgments are always based on evaluating model-generated outputs.

\noindent\textbf{Pairwise Factor Comparison.} For each factor $f_k$, we define a function $M_k$ to compare factor's manifestation in pairs of responses:
    \[
    M_k: \mathcal{R} \times \mathcal{R} \to \{-1, 0, 1\}
    \]
    Specifically, $M_k(r_i, r_j) = 1$ if factor $f_k$ is more manifest in response $r_i$; $M_k(r_i, r_j) = -1$ if factor $f_k$ is more manifest in response $r_j$; and $M_k(r_i, r_j) = 0$ if factor $f_k$ is equally manifest in both responses. For example, if $f_k$ represents length and $r_i$ is longer than $r_j$,  $M_{length}(r_i, r_j) = 1$.


% This function captures the model's explicit preferences when comparing responses directly, similar to preference labeling approaches used in studies like \citet{Lee2023RLAIFVR}.


% \paragraph{Model Preferences in Evaluation} 
% We define model preferences in an evaluation setting through pairwise comparisons.
% % We investigate model preferences during evaluation by prompting models to perform pairwise comparisons.  
% Given two responses $r_i$ and $r_j$, the model predicts a better response $P(r_i, r_j)$. 
% % We then analyze the factors present in the preferred responses (i.e., those for which $P(r_i, r_j) = 1$) across multiple pairwise comparisons.  
% % By observing which factors are consistently present in the preferred responses, we can infer the model's factor-level preferences. 
% This approach, where models make pairwise comparisons, is similar to how LLMs generate preference labels, as described in \citet{Lee2023RLAIFVR}.



% To investigate how the model expresses its preferences during generation, we prompt the model to generate a set of responses $\mathcal{R}_s = \{r | S(r) = s\}$ for each score level $s \in \{1, 2, 3, 4, 5\}$, where $S(r)$ be the score assigned by a model to a response $r$. We hypothesize that factors preferred by the model will be more prominent in higher-scoring responses (larger $s$), while less preferred factors will be more evident in lower-scoring responses (smaller $s$). This approach is inspired by methods used in constructing training data for evaluator models (e.g., ~\citet{kim2023prometheus}).
% We investigate whether models can capture and reflect such human preferences in both generation and evaluation by comparing the respective \textit{factor-level preferences} exhibited in each setting.


% \subsection{Experimental Overview: Analyzing Preferences in Generation and Evaluation}
% \label{sec:pre-exp}
% To answer our research question, we leverage the preference definitions outlined above to establish an experimental framework that analyzes both overall and factor-level pairwise preferences in both generation and evaluation settings.
% \paragraph{Model Preferences in Generation} To investigate how the model expresses its preferences during generation, we prompt the model to generate a set of responses $\mathcal{R}_s = \{r | S(r) = s\}$ for each score level $s \in \{1, 2, 3, 4, 5\}$, where $S(r)$ be the score assigned by a model to a response $r$. We hypothesize that factors preferred by the model will be more prominent in higher-scoring responses (larger $s$), while less preferred factors will be more evident in lower-scoring responses (smaller $s$). This approach is inspired by methods used in constructing training data for evaluator models (e.g., ~\citet{kim2023prometheus}).

% \paragraph{Model Preferences in Evaluation} We investigate model preferences during evaluation by prompting models to perform pairwise comparisons.  Given two responses $r_i$ and $r_j$, the model predicts a preference $P(r_i, r_j)$. We analyze the factors present in the preferred responses (i.e., those for which $P(r_i, r_j) = 1$) across multiple pairwise comparisons.  By observing which factors are consistently present in the preferred responses, we can infer the model's implicit preferences.  This approach, where models make pairwise comparisons, is similar to how LLMs generate preference labels, as described in \citet{Lee2023RLAIFVR}.




% These correlation metrics provide a robust way to assess the alignment of human and model preferences, particularly when dealing with ranking data, as in our case.

% We utilize variants of Kendall's tau [ref] to calculate the correlation between overall and factor-level pairwise preferences within each agent and the inter-agent preference alignment. Further details regarding our specific application of these metrics are provided in Section \ref{sec:profile-metric}.

% Kendall's Tau is a non-parametric measure of correlation that assesses the strength and direction of association between two variables. It is based on the ranks of data rather than their actual values, making it robust to outliers and non-normal distributions.

% \paragraph{Equation of Tau-14 and Tau-b:}
% \begin{equation}
%     \tau_{14} \textstyle= \frac{(C - D)}{( C + D + T_x)}, \quad \tau_b \textstyle= \frac{(C - D)}{\sqrt{(C + D + T_x)(C + D + T_y)}}
% \end{equation}
% where \(C\) is the number of concordant pairs, \(D\) is the number of discordant pairs, and \(T_x\) is the number of ties in the ranks of the variable \math{x}.

==> Text/archive/4_PROFILE.tex <==
Human preference is multifaceted, influenced by many factors such as fluency, helpfulness, and output length. To better understand preference alignment between humans and models, we introduce PROFILE, a novel method that automatically quantifies how these factors influence both human and model preferences.
% To this end, we introduce PROFILE, a novel method for automatically quantifying specific factors' influence on human and model preferences, revealing \textit{factor-level preferences}. 
Building on the work of \citet{hu-etal-2023-decipherpref}, PROFILE reveals factor-level preferences that help explain when and why human and model preferences align or diverge.

% PROFILE extends this analysis to assess preference alignment between humans and models by identifying the driving factors behind these preferences. 

\subsection{Operational Definitions}
We determine factor-level preferences by analyzing observable response-level preferences in a pairwise comparison setting. This setting refers to a scenario where an agent compares two responses, e.g., $r_i$ and $r_j$, and selects the preferred one (either $r_i$, $r_j$, or a tie).

To gain a comprehensive understanding of preference alignment, we analyze model preferences in two distinct settings: generation and evaluation. In the \textit{generation} setting, we examine how models internally prioritize factors when creating responses. This reveals the underlying biases and priorities embedded within the model itself. In the \textit{evaluation} setting, we observe how models judge the outcomes of different factor combinations. This reflects the model's assessment of overall response quality. 
% Comparing preferences across these two settings provides a more complete picture of model behavior and its alignment with human values. 

\paragraph{Pairwise Preferences.} 
We define the pairwise preference function for a pair of two responses as:
\[
Pref: \mathcal{R} \times \mathcal{R} \to \{1, 0, -1\},
\]
where $Pref(r_i, r_j) = 1$ if response $r_i$ is preferred over response $r_j$; $Pref(r_i, r_j) = -1$ if response $r_j$ is preferred over response $r_i$; and $Pref(r_i, r_j) = 0$ if the preference between $r_i$ and $r_j$ is a tie.

\paragraph{Generation Preferences of Language Model.}  We define a model's generation preference based on the scores it assigns to the responses. If a model scores response \(r_i\) higher than \(r_j\), it ``prefers'' \(r_i\).  We prompt the model to generate responses for scores 1-5 \((\mathcal{R} = {r_{\text{score}} \mid \text{score} \in {1, 2, 3, 4, 5} })\). 
Generation preference, \(Pref_{gen}\), is defined by comparing the model-assigned scores \(Score(r_i)\) and \(Score(r_j)\).
\(Pref_{gen}(r_i, r_j)\) is 1 if \(Score(r_i) > Score(r_j)\), and $-1$ if \(Score(r_i) < Score(r_j)\). 
This approach is inspired by methods used in constructing training
data for evaluator model~\citep{kim2023prometheus}.

\paragraph{Evaluation Preferences of Language Model.}  We define evaluation preference by having the model directly compare two responses. Evaluation preference, \(Pref_{eval}(r_i, r_j)\), is $1$ if the model prefers \(r_i\), $-1$ if it prefers \(r_j\), and $0$ if they are equally preferable. This pairwise evaluation approach is similar to how LLMs generate preference labels~\citep{Lee2023RLAIFVR}. We assume human preferences are consistent across generation and evaluation, as human judgment always involves evaluating generated outputs.

\subsection{Quantification of Human-Model Preference Alignment}
\label{sec:profile-metric}
\input{Figure/taxonomy}
This section outlines the process of quantifying \textit{factor-level preferences} and measuring the alignment of these preferences between humans and the model. First, we calculate \textit{factor score} \(f(\mathcal{R})\) by comparing the pairwise preference (\(Pref\)) with the factor-specific pairwise comparison (\(M_k\)) across the set of all possible response pairs in the dataset. These scores are then used to rank the factors, and the alignment between human and model preferences at the factor level is quantitatively evaluated based on these rankings.

\paragraph{Factor Taxonomy.} 
\label{sec:factor_taxonomy}
To provide a structured framework for analyzing preferences across a wide range of criteria, we develop a unified taxonomy of fine-grained factors relevant to text quality. This taxonomy systematically categorizes the factors influencing preference alignment between humans and AI models across text generation tasks. Addressing the lack of a unified framework and inconsistent terminology in existing literature, we consolidate evaluation factors from diverse tasks, including summarization, helpful response generation, question answering, and instruction following. For summarization-specific factors, we draw from~\citet{fu2024gptscore, hu-etal-2023-decipherpref, zhong-etal-2022-towards, fabbri2021summeval}. For helpfulness and document-based question answering, we incorporate categories from \citet{glaese2022improving, ye2024flask, nakano2021webgpt}. The complete taxonomy is detailed in Table~\ref{tab:taxonomy}.

\paragraph{Automatically Determining Factor Manifestation.}
% \paragraph{Pairwise Factor Comparisons.}  
For each factor $f_k$, we define a function $M_k$ to compare factor's manifestation in pairs of responses:
\[M_k: \mathcal{R} \times \mathcal{R} \to \{-1, 0, 1\}\]
Specifically, $M_k(r_i, r_j) = 1$ if factor $f_k$ is more manifest in response $r_i$; $M_k(r_i, r_j) = -1$ if factor $f_k$ is more manifest in response $r_j$; and $M_k(r_i, r_j) = 0$ if factor $f_k$ is equally manifest in both responses.

We employ several approaches to automatically determine factor manifestation $M_k$, depending on the factor's nature: (i) \textbf{Rule-based}: For straightforward, objective factors, we use deterministic algorithms. $\mathsf{Length}$ and $\mathsf{Novel\:Words}$ are extracted this way. (ii) \textbf{UniEval-based}: For inherently subjective factors ($\mathsf{Fluency}$ and $\mathsf{Coherence}$), we use the well-established UniEval metric~\citep{zhong-etal-2022-towards}. UniEval is a learned metric that provides scores of range 0-1 for various aspects of text quality. 
(iii) \textbf{LLM-based}: For factors that rely on objective criteria but require more nuanced judgment, we use GPT-4o with carefully designed prompts. This approach is further divided into ``response-based'' ($\mathsf{Intent\:Alignment}$ and $\mathsf{Formality\:Alignment}$) and ``atomic-fact-based'' (the remaining seven) extraction depending on the level of detail needed for each factor.
The specific details of the implementation of each method and validation of LLM-based extractions can be found in Appendix~\ref{sec:appendix_profile}.

% To analyze the manifestation of our factors in model and human-preferred responses and 
% determine $M_k$, we develop an automatic factor extraction framework. We employ three approaches based on the objectivity of each factor:
% (i) Rule-based: For straightforward, objective factors, we use deterministic algorithms. $\mathsf{Length}$ and $\mathsf{Novel\:Words}$ are extracted this way. (ii) UniEval-based: For inherently subjective factors ($\mathsf{Fluency}$ and $\mathsf{Coherence}$), we use the well-established UniEval metric~\citep{zhong-etal-2022-towards}. UniEval is a learned metric that provides scores of range 0-1 for various aspects of text quality. 
% (iii) LLM-based: For factors that rely on objective criteria but require more nuanced judgment, we use GPT-4o with carefully designed prompts. This approach is further divided into ``response-based'' ($\mathsf{Intent\:Alignment}$ and $\mathsf{Formality\:Alignment}$) and ``atomic-fact-based'' (the remaining seven) extraction depending on the level of detail needed for each factor.
% By combining these three approaches, our framework captures a wide range of factors with appropriate levels of objectivity.
% The specific details of the implementation of each method and validation of LLM-based extractions can be found in Appendix~\ref{sec:appendix_profile}.

\paragraph{Quantifying Influence of Each Factor.}
% Response pair $r_i$와 $r_j$에 대해서 그 response-level/overall preference (Pref)와 the manifestation of factor \(f_k\) in the response가 일치하는지 여부 (concordance)를 바탕으로 각 factor의 influence를 측정한다. 
To quantify each factor's influence (factor score), we analyze the concordance between response-level preferences $(Pref(r_i, r_j))$ and factor manifestation \((M_k(r_i, r_j))\) across response pairs. 
% For a given factor $f_k$, we measure whether the overall preference aligns with how that factor manifests in the responses. 
We use $\tau_{14}$, a variation of Kendall's correlation proposed by~\citet{deutsch-etal-2023-ties}, which is particularly well-suited for handling ties in our analysis setting, where ties arise in only one of the comparison sets used for calculating Kendall’s \(\tau\). 

% To {quantify the influence of each factor, i.e., \textit{factor score}, we use \(\tau_{14}\), a variation of Kendall's correlation proposed by~\citet{deutsch-etal-2023-ties}.}
% This metric is well-suited for handling the distribution of ties, particularly in our setting, where ties arise in only one of the comparison sets used for calculating Kendall’s \(\tau\). 
% Below, we explain the specific ways ties appear in our analysis.}

% Since our analysis relies on pairwise comparisons, we calculate \(\tau_{14}\) for each factor $f_k$ using pairwise concordance and discordance, following the methodology outlined by~\citet{bojar-etal-2017-results}. 

The metric is defined as:
\begin{equation} \label{eq:factorscore}
\tau_{14}(f_k) = \frac{|C_k| - |D_k|}{|C_k| + |D_k| + |T_k|,}
\end{equation}
where \(C_k\) is the count of concordant pairs (preference and factor manifestation agree), \(D_k\) is the count of discordant pairs (preference and factor manifestation disagree), and \(T_k\) represents ties. 

The definition of \(T_k\) varies by setting: (1) In the \textbf{generation} setting, since models don't generate responses with identical scores, \(T_k\) only counts factor-level ties ($M_k(r_i, r_j) = 0$). (2) In the \textbf{evaluation} setting, we remove factor-level ties for clearer analysis, so \(T_k\) counts only preference-level ties $(Pref(r_i, r_j) = 0)$.

For instance, consider the factor \(M_{length}\), which measures response length. If response \(r_1\) is longer than \(r_2\) (\(M_{length}(r_1, r_2) = 1\)) and the model prefers \(r_1\) (\(Pref(r_1, r_2) = 1\)), this pair is classified as concordant. Conversely, if the model prefers the shorter \(r_1\), the pair is discordant. Evaluating all pairs, a positive factor score indicates a positive influence of the factor, a negative score indicates a negative influence, and a score close to zero implies minimal influence. The magnitude of the score reflects the strength of this influence.

% The calculation of factor score differs between generation and evaluation settings. In generation, \(T_k\) counts ties at the factor level ($M_k(r_i, r_j) = 0$), as there are no ties in model-generated scores. In evaluation, we remove ties at the preference level $Pref(r_i, r_j) = tie$ before calculating \(\tau_{14}\), focusing solely on the influence of the factor where a preference exists.

% Gen, Eval different definitions
% Crucially, the definition of \(T_k\) differs between generation and evaluation settings.  In generation, \(T_k\) counts ties at the factor level ($M_k(r_i, r_j) = 0$), as there are no ties in model-generated scores. In evaluation, we remove ties at the preference level $Pref(r_i, r_j) = tie$ before calculating \(\tau_{14}\), focusing solely on the influence of the factor where a preference exists.
% where \(C_k\) is the count of concordant pairs, where the overall preference and the manifestation of factor \(f_k\) agree, \(D_k\) is the count of discordant pairs, where the overall preference and the manifestation of factor \(f_k\) disagree, and \(T_k\) is the count of ties, are handled differently depending on the context. Mathematically, \(C_k\) and \(D_k\) are computed as:
% \[
% C_k \textstyle= \sum_{r_i, r_j \in R, i<j} \mathbbm{1}[Pref(r_i, r_j) \cdot M_k(r_i, r_j) = +1],\]
% \[
% D_k \textstyle= \sum_{r_i, r_j \in R, i<j} \mathbbm{1}[Pref(r_i, r_j) \cdot M_k(r_i, r_j) = -1], 
% \]
% \[
% T_k \textstyle= \sum_{r_i, r_j \in R, i<j} 
% \begin{cases} 
% \mathbb{1}[M_k(r_i, r_j) = 0] & \text{in generation setting} \\
% \mathbb{1}[Pref(r_i, r_j) = 0] & \text{in evaluation setting}
% \end{cases}
% \]
% where \(\mathbbm{1}[\text{condition}]\) is 1 if the condition is true and 0 otherwise. 

\paragraph{Evaluating Factor-Level Preference Alignment.}
Finally, we evaluate \textit{factor-level preference} alignment by comparing human and model factor rankings.  We use Spearman’s \(\rho\), Kendall’s \(\tau\)~\footnote{We use Kendall's $\tau_b$~\citep{kendall1945treatment} as the default.}, and Pearson’s \(r\) coefficients to quantify the correlation between these rankings, providing a measure of how well the model's factor priorities align with human values.

% An agent's \textit{factor-level preferences} are defined as a ranking of factors based on their scores, where a higher rank and score indicate a stronger influence of that factor on the agent's overall preference. The correlation between human and model rankings reflects their agreement on the relative importance of factors to overall preference, which we use as a measure of factor-level preference alignment between humans and models. We calculate Spearman's \(\rho\), Kendall's \(\tau\)~\footnote{We use Kendall's $\tau_b$~\citep{kendall1945treatment} as the default.}, and Pearson's \(r\) coefficients to quantify this alignment.
% We assume human preferences are consistent across generation and evaluation tasks since human judgments are always based on evaluating model-generated outputs.


